Rediscovering Bottom-Up: Effective Forecasting in Temporal Hierarchies

Forecast reconciliation has become a prominent topic in recent forecasting literature, with a primary distinction made between cross-sectional and temporal hierarchies. This work focuses on temporal hierarchies, such as aggregating monthly time series data to annual data. We explore the impact of various forecast reconciliation methods on temporally aggregated ARIMA models, thereby bridging the fields of hierarchical forecast reconciliation and temporal aggregation both theoretically and experimentally. Our paper is the first to theoretically examine the effects of temporal hierarchical forecast reconciliation, demonstrating that the optimal method aligns with a bottom-up aggregation approach. To assess the practical implications and performance of the reconciled forecasts, we conduct a series of simulation studies, confirming that the findings extend to more complex models. This result helps explain the strong performance of the bottom-up approach observed in many prior studies. Finally, we apply our methods to real data examples, where we observe similar results.

==> tables/h=1,k=1,12,sigma.sq=1,auto=FALSE.tex <==
\begin{table}
\centering
\caption{\label{tab:h=1, k=(1,12), sigma.sq=1, auto=FALSE}Mean rMSE per buckets of $\phi$ for $ h=1, k\in\{12,1\}, \sigma^2=1 $ and fixed order of the used models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrrr}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{3}{c}{Training rMSE} & \multicolumn{3}{c}{Test rMSE} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9}
Level & n & Recon. Type & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9] & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9]\\
\midrule
 &  & Bottom-Up & 0.15 (0.02) & 0.21 (0.01) & 0.07 (0.02) & \textbf{-0.14 (0.03)} & \textbf{-0.08 (0.02)} & \textbf{-0.11 (0.02)}\\

 &  & Full Cov. & \textbf{-0.03 (0.01)} & 0.04 (0.02) & \textbf{-0.07 (0.01)} & 0.01 (0.02) & 0.10 (0.03) & 0.03 (0.06)\\

 &  & Spectral & -0.02 (0.00) & 0.02 (0.00) & -0.03 (0.01) & -0.05 (0.01) & -0.03 (0.01) & -0.01 (0.03)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.01 (0.00) & \textbf{ 0.00 (0.00)} & -0.01 (0.00) & -0.03 (0.00) & -0.02 (0.00) & -0.03 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.01) & 0.07 (0.00) & -0.05 (0.01) & \textbf{-0.08 (0.01)} & \textbf{-0.06 (0.01)} & \textbf{-0.13 (0.01)}\\

 &  & Full Cov. & \textbf{-0.05 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.09 (0.01)} & -0.04 (0.01) & 0.01 (0.00) & -0.09 (0.01)\\

 &  & Spectral & -0.04 (0.00) & 0.00 (0.00) & -0.08 (0.01) & -0.04 (0.01) & -0.01 (0.01) & -0.09 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.01 (0.00) & 0.00 (0.00) & -0.02 (0.00) & -0.02 (0.00) & -0.01 (0.00) & -0.02 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.03 (0.00) & 0.02 (0.00) & -0.09 (0.01) & \textbf{-0.09 (0.01)} & \textbf{-0.03 (0.00)} & \textbf{-0.13 (0.01)}\\

 &  & Full Cov. & \textbf{-0.05 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.10 (0.01)} & -0.06 (0.01) & 0.00 (0.00) & -0.11 (0.01)\\

 &  & Spectral & -0.04 (0.00) & 0.00 (0.00) & -0.10 (0.01) & -0.06 (0.01) & -0.01 (0.00) & -0.11 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & -0.01 (0.00) & 0.00 (0.00) & -0.02 (0.00) & -0.01 (0.00) & -0.01 (0.00) & -0.02 (0.00)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.05 (0.01)} & -0.03 (0.02) & \textbf{-0.07 (0.00)} & 0.17 (0.02) & 0.23 (0.02) & 0.20 (0.03)\\

 &  & Spectral & -0.02 (0.00) & \textbf{-0.03 (0.00)} & -0.03 (0.01) & 0.01 (0.00) & 0.05 (0.01) & 0.19 (0.07)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & -0.01 (0.00) & 0.00 (0.01) & 0.01 (0.00) & 0.02 (0.00) & 0.13 (0.02)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.02 (0.00)} & \textbf{-0.03 (0.00)} & \textbf{-0.03 (0.00)} & 0.04 (0.00) & 0.06 (0.01) & 0.04 (0.01)\\

 &  & Spectral & -0.01 (0.00) & -0.01 (0.00) & -0.01 (0.00) & 0.01 (0.01) & 0.03 (0.01) & 0.04 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & -0.01 (0.00) & 0.03 (0.01) & 0.00 (0.00) & 0.01 (0.00) & 0.09 (0.01)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.01 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.01 (0.00)} & 0.02 (0.00) & 0.02 (0.00) & 0.01 (0.00)\\

 &  & Spectral & -0.01 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.00) & 0.01 (0.00) & 0.01 (0.00)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.04 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.07 (0.01)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.09 (0.01) & 0.18 (0.01) & 0.07 (0.02) & \textbf{-0.12 (0.02)} & \textbf{-0.09 (0.01)} & \textbf{-0.11 (0.02)}\\

 &  & Full Cov. & \textbf{-0.04 (0.00)} & 0.04 (0.02) & \textbf{-0.07 (0.01)} & 0.04 (0.02) & 0.11 (0.02) & 0.03 (0.06)\\

 &  & Spectral & -0.02 (0.00) & 0.01 (0.00) & -0.03 (0.01) & -0.04 (0.01) & -0.03 (0.01) & -0.01 (0.03)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & -0.01 (0.00) & -0.02 (0.00) & -0.02 (0.00) & -0.03 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.06 (0.00) & -0.05 (0.01) & \textbf{-0.06 (0.01)} & \textbf{-0.05 (0.01)} & \textbf{-0.13 (0.01)}\\

 &  & Full Cov. & \textbf{-0.04 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.09 (0.01)} & -0.02 (0.01) & 0.02 (0.00) & -0.09 (0.01)\\

 &  & Spectral & -0.03 (0.00) & 0.00 (0.00) & -0.08 (0.01) & -0.02 (0.00) & -0.01 (0.00) & -0.09 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.01 (0.00) & 0.00 (0.00) & -0.01 (0.00) & -0.01 (0.00) & -0.01 (0.00) & -0.02 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.02 (0.00) & 0.02 (0.00) & -0.08 (0.01) & \textbf{-0.07 (0.01)} & \textbf{-0.03 (0.00)} & \textbf{-0.13 (0.01)}\\

 &  & Full Cov. & \textbf{-0.04 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.10 (0.01)} & -0.04 (0.00) & 0.00 (0.00) & -0.11 (0.01)\\

 &  & Spectral & -0.03 (0.00) & 0.00 (0.00) & -0.09 (0.01) & -0.04 (0.00) & -0.01 (0.00) & -0.10 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & -0.01 (0.00) & 0.00 (0.00) & -0.02 (0.00) & -0.01 (0.00) & -0.01 (0.00) & -0.02 (0.00)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=1,k=1,12,sigma.sq=1,auto=TRUE.tex <==
\begin{table}
\centering
\caption{\label{tab:h=1, k=(1,12), sigma.sq=1, auto=TRUE}Mean rMSE per buckets of $\phi$ for $ h=1, k\in\{12,1\}, \sigma^2=1 $ and auto-selected models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrrr}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{3}{c}{Training rMSE} & \multicolumn{3}{c}{Test rMSE} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9}
Level & n & Recon. Type & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9] & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9]\\
\midrule
 &  & Bottom-Up & 0.02 (0.01) & 0.04 (0.01) & 0.06 (0.03) & \textbf{-0.06 (0.02)} & \textbf{-0.02 (0.01)} & 0.00 (0.04)\\

 &  & Full Cov. & \textbf{-0.09 (0.01)} & - & \textbf{-0.14 (0.01)} & 0.04 (0.03) & - & -0.02 (0.03)\\

 &  & Spectral & -0.05 (0.01) & \textbf{-0.02 (0.00)} & -0.11 (0.01) & -0.04 (0.01) & -0.01 (0.01) & -0.02 (0.03)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.01 (0.00) & 0.00 (0.00) & -0.02 (0.00) & -0.02 (0.00) & -0.01 (0.00) & \textbf{-0.03 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.03 (0.01) & 0.02 (0.00) & -0.01 (0.01) & \textbf{-0.09 (0.01)} & \textbf{-0.03 (0.01)} & -0.03 (0.02)\\

 &  & Full Cov. & \textbf{-0.07 (0.00)} & - & \textbf{-0.11 (0.01)} & -0.06 (0.01) & - & \textbf{-0.06 (0.01)}\\

 &  & Spectral & -0.05 (0.00) & \textbf{-0.01 (0.00)} & -0.09 (0.01) & -0.05 (0.01) & -0.01 (0.00) & -0.04 (0.02)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.01 (0.00) & 0.00 (0.00) & -0.02 (0.00) & -0.01 (0.00) & -0.01 (0.00) & -0.02 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.03 (0.01) & 0.08 (0.02) & 0.00 (0.02) & \textbf{-0.07 (0.01)} & 0.04 (0.02) & -0.03 (0.02)\\

 &  & Full Cov. & \textbf{-0.06 (0.00)} & - & \textbf{-0.10 (0.01)} & -0.06 (0.01) & - & \textbf{-0.09 (0.01)}\\

 &  & Spectral & -0.05 (0.00) & \textbf{-0.01 (0.00)} & -0.09 (0.01) & -0.05 (0.00) & \textbf{-0.01 (0.00)} & -0.08 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & -0.01 (0.00) & 0.00 (0.00) & -0.02 (0.00) & -0.01 (0.00) & 0.00 (0.00) & -0.02 (0.00)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.06 (0.00)} & - & \textbf{-0.09 (0.01)} & 0.11 (0.02) & - & 0.09 (0.02)\\

 &  & Spectral & -0.02 (0.00) & \textbf{-0.01 (0.00)} & -0.05 (0.01) & 0.01 (0.00) & 0.01 (0.00) & 0.06 (0.01)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.01) & 0.00 (0.00) & 0.01 (0.00) & 0.10 (0.02)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.03 (0.00)} & - & \textbf{-0.06 (0.01)} & 0.04 (0.01) & - & 0.01 (0.01)\\

 &  & Spectral & -0.01 (0.00) & \textbf{-0.01 (0.00)} & -0.03 (0.01) & 0.01 (0.00) & 0.01 (0.00) & 0.01 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.01) & 0.00 (0.00) & 0.00 (0.00) & 0.04 (0.01)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & 0.00 (0.00) & 0.00 (0.00)\\

 &  & Full Cov. & \textbf{-0.01 (0.00)} & - & \textbf{-0.05 (0.01)} & 0.02 (0.00) & - & \textbf{-0.01 (0.01)}\\

 &  & Spectral & -0.01 (0.00) & \textbf{-0.01 (0.00)} & -0.04 (0.01) & 0.01 (0.00) & 0.00 (0.00) & -0.01 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & -0.01 (0.00) & 0.01 (0.01) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & 0.03 (0.01)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.01 (0.01) & 0.04 (0.01) & 0.05 (0.03) & \textbf{-0.05 (0.01)} & \textbf{-0.02 (0.01)} & -0.01 (0.04)\\

 &  & Full Cov. & \textbf{-0.08 (0.01)} & - & \textbf{-0.14 (0.01)} & 0.04 (0.02) & - & -0.03 (0.03)\\

 &  & Spectral & -0.04 (0.00) & \textbf{-0.01 (0.00)} & -0.11 (0.01) & -0.02 (0.01) & -0.01 (0.00) & -0.02 (0.03)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.01 (0.00) & 0.00 (0.00) & -0.02 (0.00) & -0.01 (0.00) & -0.01 (0.00) & \textbf{-0.03 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.02 (0.00) & 0.02 (0.00) & -0.01 (0.01) & \textbf{-0.06 (0.01)} & \textbf{-0.03 (0.01)} & -0.03 (0.02)\\

 &  & Full Cov. & \textbf{-0.06 (0.00)} & - & \textbf{-0.11 (0.01)} & -0.03 (0.01) & - & \textbf{-0.06 (0.01)}\\

 &  & Spectral & -0.04 (0.00) & \textbf{-0.01 (0.00)} & -0.08 (0.01) & -0.03 (0.00) & -0.01 (0.00) & -0.04 (0.02)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.01 (0.00) & 0.00 (0.00) & -0.02 (0.00) & -0.01 (0.00) & 0.00 (0.00) & -0.02 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.02 (0.01) & 0.08 (0.02) & 0.00 (0.02) & \textbf{-0.05 (0.01)} & 0.04 (0.02) & -0.03 (0.02)\\

 &  & Full Cov. & \textbf{-0.05 (0.00)} & - & \textbf{-0.10 (0.01)} & -0.04 (0.00) & - & \textbf{-0.09 (0.01)}\\

 &  & Spectral & -0.04 (0.00) & \textbf{-0.01 (0.00)} & -0.09 (0.01) & -0.03 (0.00) & \textbf{-0.01 (0.00)} & -0.08 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & -0.01 (0.00) & 0.00 (0.00) & -0.02 (0.00) & -0.01 (0.00) & 0.00 (0.00) & -0.02 (0.00)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=1,k=1,4,12,sigma.sq=1,auto=FALSE,name=test_rel_err.tex <==
\begin{table}
\centering
\caption{\label{tab:h=1, k=(1,4,12), sigma.sq=1, auto=FALSE, name=test_rel_err}Test mean rMSE per buckets of $\phi$ for $ h=1, k=(1,4,12), \sigma^2=1 $ and fixed order of the used models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrr}
\toprule
Level & n & Recon. Type & {}[-0.9,-0.6] & (-0.6,-0.3] & (-0.3,0.3] & (0.3,0.6] & (0.6,0.9]\\
\midrule
 &  & Bottom-Up & -0.035 (0.031) & -0.066 (0.064) & -0.061 (0.019) & -0.053 (0.033) & -0.004 (0.069)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.036 (0.013) & -0.033 (0.020) & -0.034 (0.010) & -0.018 (0.024) & 0.013 (0.050)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.057 (0.007) & -0.057 (0.010) & -0.039 (0.005) & -0.053 (0.007) & -0.064 (0.012)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.086 (0.015) & -0.053 (0.015) & -0.053 (0.010) & -0.078 (0.014) & -0.155 (0.020)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.054 (0.011) & -0.034 (0.008) & -0.030 (0.005) & -0.051 (0.009) & -0.129 (0.017)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.042 (0.004) & -0.022 (0.004) & -0.025 (0.003) & -0.033 (0.004) & -0.070 (0.006)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.100 (0.009) & -0.083 (0.016) & -0.033 (0.005) & -0.046 (0.008) & -0.154 (0.015)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.065 (0.006) & -0.043 (0.009) & -0.020 (0.003) & -0.029 (0.006) & -0.149 (0.013)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & -0.039 (0.003) & -0.029 (0.006) & -0.014 (0.002) & -0.020 (0.002) & -0.062 (0.004)\\
\cmidrule{1-8}
 &  & Bottom-Up & -0.045 (0.009) & -0.034 (0.008) & -0.014 (0.004) & -0.033 (0.006) & -0.042 (0.011)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & 0.009 (0.009) & 0.031 (0.010) & 0.027 (0.009) & 0.071 (0.023) & 0.030 (0.018)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.012 (0.005) & 0.012 (0.007) & 0.016 (0.005) & 0.037 (0.012) & 0.073 (0.029)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.052 (0.005) & -0.018 (0.003) & -0.011 (0.003) & -0.027 (0.003) & -0.036 (0.006)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.015 (0.005) & -0.004 (0.002) & 0.011 (0.004) & 0.011 (0.010) & 0.000 (0.011)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.014 (0.002) & -0.002 (0.002) & 0.010 (0.004) & 0.020 (0.008) & 0.074 (0.018)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.050 (0.004) & -0.015 (0.003) & -0.005 (0.001) & -0.016 (0.002) & -0.040 (0.004)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.031 (0.003) & 0.025 (0.025) & 0.003 (0.002) & -0.005 (0.003) & -0.031 (0.004)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & -0.015 (0.002) & 0.018 (0.013) & 0.004 (0.002) & 0.003 (0.002) & 0.048 (0.008)\\
\cmidrule{1-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & 0.036 (0.009) & 0.023 (0.006) & 0.027 (0.005) & 0.081 (0.017) & 0.078 (0.019)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.006 (0.001) & 0.009 (0.002) & 0.012 (0.003) & 0.045 (0.008) & 0.113 (0.028)\\
\cmidrule{2-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & 0.017 (0.003) & 0.004 (0.001) & 0.013 (0.003) & 0.026 (0.007) & 0.032 (0.008)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.006 (0.001) & 0.003 (0.001) & 0.008 (0.002) & 0.030 (0.006) & 0.097 (0.015)\\
\cmidrule{2-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & 0.007 (0.001) & 0.013 (0.009) & 0.003 (0.001) & 0.008 (0.002) & 0.009 (0.003)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 3} & \multirow{-4}{*}{ 100} & OLS & 0.005 (0.000) & 0.007 (0.003) & 0.003 (0.001) & 0.012 (0.002) & 0.078 (0.009)\\
\cmidrule{1-8}
 &  & Bottom-Up & -0.064 (0.015) & -0.101 (0.025) & -0.062 (0.014) & -0.080 (0.022) & -0.051 (0.047)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.020 (0.007) & -0.027 (0.012) & -0.029 (0.007) & -0.023 (0.019) & -0.016 (0.037)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.038 (0.003) & -0.041 (0.005) & -0.032 (0.003) & -0.048 (0.005) & -0.066 (0.008)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.072 (0.008) & -0.043 (0.010) & -0.047 (0.008) & -0.074 (0.012) & -0.149 (0.018)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.035 (0.005) & -0.024 (0.005) & -0.023 (0.004) & -0.045 (0.008) & -0.122 (0.016)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.028 (0.002) & -0.016 (0.003) & -0.019 (0.002) & -0.028 (0.003) & -0.061 (0.005)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.066 (0.006) & -0.066 (0.014) & -0.027 (0.004) & -0.042 (0.007) & -0.145 (0.013)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.040 (0.003) & -0.031 (0.007) & -0.015 (0.002) & -0.025 (0.005) & -0.140 (0.012)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & -0.023 (0.002) & -0.021 (0.005) & -0.010 (0.001) & -0.016 (0.002) & -0.054 (0.003)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=1,k=1,4,12,sigma.sq=1,auto=FALSE,name=train_rel_err.tex <==
\begin{table}
\centering
\caption{\label{tab:h=1, k=(1,4,12), sigma.sq=1, auto=FALSE, name=train_rel_err}Training mean rMSE per buckets of $\phi$ for $ h=1, k=(1,4,12), \sigma^2=1 $ and fixed order of the used models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrr}
\toprule
Level & n & Recon. Type & {}[-0.9,-0.6] & (-0.6,-0.3] & (-0.3,0.3] & (0.3,0.6] & (0.6,0.9]\\
\midrule
 &  & Bottom-Up & 0.148 (0.019) & 0.189 (0.024) & 0.180 (0.012) & 0.181 (0.018) & 0.024 (0.022)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.035 (0.006) & -0.007 (0.006) & 0.018 (0.004) & -0.022 (0.009) & -0.121 (0.016)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.003 (0.003) & 0.010 (0.003) & 0.014 (0.001) & 0.008 (0.002) & -0.036 (0.005)\\
\cmidrule{2-8}
 &  & Bottom-Up & 0.004 (0.009) & 0.048 (0.008) & 0.065 (0.004) & 0.046 (0.006) & -0.098 (0.013)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.049 (0.005) & -0.010 (0.005) & 0.002 (0.002) & -0.014 (0.003) & -0.144 (0.010)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.015 (0.002) & 0.000 (0.001) & 0.003 (0.000) & -0.001 (0.001) & -0.050 (0.003)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.040 (0.005) & 0.016 (0.006) & 0.028 (0.002) & 0.004 (0.004) & -0.145 (0.009)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.057 (0.003) & -0.018 (0.003) & 0.001 (0.001) & -0.022 (0.003) & -0.161 (0.009)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & -0.019 (0.001) & -0.002 (0.001) & 0.001 (0.000) & -0.006 (0.001) & -0.058 (0.003)\\
\cmidrule{1-8}
 &  & Bottom-Up & -0.018 (0.006) & 0.005 (0.004) & 0.020 (0.002) & 0.005 (0.003) & -0.028 (0.006)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.077 (0.006) & -0.061 (0.006) & -0.037 (0.003) & -0.083 (0.006) & -0.114 (0.009)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.030 (0.002) & -0.026 (0.003) & -0.024 (0.002) & -0.042 (0.003) & -0.027 (0.009)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.041 (0.003) & -0.004 (0.002) & 0.005 (0.001) & -0.007 (0.002) & -0.037 (0.004)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.056 (0.003) & -0.024 (0.002) & -0.019 (0.001) & -0.037 (0.002) & -0.069 (0.005)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.024 (0.001) & -0.013 (0.001) & -0.011 (0.001) & -0.020 (0.001) & 0.012 (0.006)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.046 (0.003) & -0.009 (0.001) & 0.001 (0.000) & -0.012 (0.001) & -0.038 (0.003)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.052 (0.003) & -0.020 (0.002) & -0.009 (0.001) & -0.025 (0.001) & -0.051 (0.003)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & -0.021 (0.001) & -0.009 (0.001) & -0.006 (0.000) & -0.010 (0.001) & 0.035 (0.005)\\
\cmidrule{1-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.042 (0.004) & -0.038 (0.005) & -0.028 (0.002) & -0.061 (0.005) & -0.076 (0.008)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.001 (0.001) & -0.006 (0.001) & -0.013 (0.001) & -0.025 (0.003) & 0.005 (0.009)\\
\cmidrule{2-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.019 (0.002) & -0.011 (0.001) & -0.013 (0.001) & -0.021 (0.002) & -0.029 (0.004)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.002 (0.000) & -0.001 (0.000) & -0.005 (0.000) & -0.007 (0.001) & 0.045 (0.006)\\
\cmidrule{2-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.011 (0.001) & -0.007 (0.001) & -0.005 (0.000) & -0.009 (0.001) & -0.012 (0.002)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 3} & \multirow{-4}{*}{ 100} & OLS & 0.003 (0.000) & 0.000 (0.000) & -0.002 (0.000) & 0.002 (0.001) & 0.064 (0.005)\\
\cmidrule{1-8}
 &  & Bottom-Up & 0.056 (0.008) & 0.106 (0.012) & 0.123 (0.008) & 0.137 (0.014) & 0.011 (0.020)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.050 (0.005) & -0.026 (0.005) & 0.001 (0.003) & -0.036 (0.008) & -0.124 (0.015)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.010 (0.001) & -0.002 (0.001) & 0.003 (0.001) & -0.003 (0.001) & -0.038 (0.004)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.009 (0.004) & 0.029 (0.005) & 0.047 (0.003) & 0.035 (0.005) & -0.094 (0.012)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.043 (0.003) & -0.013 (0.003) & -0.004 (0.001) & -0.018 (0.003) & -0.138 (0.009)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.013 (0.001) & -0.003 (0.001) & 0.000 (0.000) & -0.005 (0.001) & -0.045 (0.002)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.032 (0.003) & 0.008 (0.004) & 0.020 (0.002) & 0.001 (0.003) & -0.135 (0.009)\\

 &  & Full Cov. & - & - & - & - & -\\

 &  & Spectral & -0.045 (0.002) & -0.017 (0.003) & -0.001 (0.001) & -0.023 (0.002) & -0.151 (0.008)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & -0.014 (0.001) & -0.003 (0.000) & -0.001 (0.000) & -0.007 (0.000) & -0.049 (0.002)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=1,k=1,4,12,sigma.sq=1,auto=FALSE.tex <==
\begin{table}
\centering
\caption{\label{tab:h=1, k=(1,4,12), sigma.sq=1, auto=FALSE}Mean rMSE per buckets of $\phi$ for $ h=1, k\in\{12,4,1\}, \sigma^2=1 $ and fixed order of the used models. The standard errors are given in parentheses.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrrr}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{3}{c}{Training rMSE} & \multicolumn{3}{c}{Test rMSE} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9}
Level & n & Recon. Type & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9] & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9]\\
\midrule
 &  & Bottom-Up & 0.16 (0.02) & 0.20 (0.01) & 0.08 (0.02) & -0.05 (0.04) & \textbf{-0.06 (0.02)} & \textbf{-0.13 (0.03)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.03 (0.01)} & \textbf{ 0.01 (0.00)} & \textbf{-0.07 (0.01)} & \textbf{-0.06 (0.01)} & 0.00 (0.01) & 0.02 (0.05)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & 0.01 (0.00) & -0.02 (0.00) & -0.05 (0.01) & -0.05 (0.00) & -0.08 (0.01)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.02 (0.01) & 0.07 (0.00) & -0.04 (0.01) & \textbf{-0.10 (0.01)} & \textbf{-0.05 (0.01)} & \textbf{-0.15 (0.01)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.04 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.09 (0.01)} & -0.04 (0.01) & 0.00 (0.01) & -0.07 (0.02)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.01 (0.00) & 0.00 (0.00) & -0.03 (0.00) & -0.05 (0.00) & -0.02 (0.00) & -0.06 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.03 (0.00) & 0.03 (0.00) & -0.08 (0.01) & \textbf{-0.08 (0.01)} & \textbf{-0.04 (0.00)} & \textbf{-0.13 (0.01)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.04 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.10 (0.01)} & -0.04 (0.01) & -0.01 (0.00) & -0.10 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & -0.02 (0.00) & 0.00 (0.00) & -0.04 (0.00) & -0.03 (0.00) & -0.02 (0.00) & -0.05 (0.00)\\
\cmidrule{1-9}
 &  & Bottom-Up & -0.02 (0.00) & 0.01 (0.00) & -0.02 (0.00) & \textbf{-0.05 (0.01)} & \textbf{-0.01 (0.00)} & \textbf{-0.04 (0.01)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.07 (0.00)} & \textbf{-0.05 (0.00)} & \textbf{-0.09 (0.01)} & 0.02 (0.01) & 0.06 (0.01) & 0.18 (0.05)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.03 (0.00) & -0.03 (0.00) & -0.04 (0.01) & 0.00 (0.01) & 0.02 (0.01) & 0.12 (0.02)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.03 (0.00) & 0.00 (0.00) & -0.02 (0.00) & \textbf{-0.04 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.04 (0.00)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.05 (0.00)} & \textbf{-0.03 (0.00)} & \textbf{-0.05 (0.00)} & 0.02 (0.01) & 0.03 (0.01) & 0.03 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.02 (0.00) & -0.01 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.00) & 0.05 (0.01)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.04 (0.00) & 0.00 (0.00) & -0.03 (0.00) & \textbf{-0.05 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.03 (0.00)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.04 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.04 (0.00)} & -0.02 (0.00) & 0.01 (0.00) & -0.01 (0.00)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & -0.02 (0.00) & -0.01 (0.00) & 0.01 (0.00) & -0.01 (0.00) & 0.01 (0.00) & 0.04 (0.01)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.03 (0.00)} & \textbf{-0.04 (0.00)} & \textbf{-0.06 (0.01)} & 0.04 (0.01) & 0.05 (0.01) & 0.19 (0.04)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & -0.02 (0.00) & -0.01 (0.01) & 0.01 (0.00) & 0.01 (0.00) & 0.14 (0.02)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.02 (0.00)} & \textbf{-0.02 (0.00)} & \textbf{-0.03 (0.00)} & 0.03 (0.01) & 0.02 (0.00) & 0.06 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & -0.01 (0.00) & 0.02 (0.00) & 0.01 (0.00) & 0.01 (0.00) & 0.07 (0.01)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.01 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.01 (0.00)} & 0.01 (0.00) & 0.01 (0.00) & 0.02 (0.00)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 3} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.03 (0.00) & 0.01 (0.00) & 0.00 (0.00) & 0.05 (0.01)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.06 (0.01) & 0.14 (0.01) & 0.06 (0.02) & \textbf{-0.09 (0.01)} & \textbf{-0.06 (0.01)} & \textbf{-0.14 (0.02)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.04 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.08 (0.01)} & -0.03 (0.01) & 0.00 (0.01) & 0.01 (0.04)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.01 (0.00) & 0.00 (0.00) & -0.03 (0.00) & -0.04 (0.00) & -0.04 (0.00) & -0.07 (0.01)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.05 (0.00) & -0.04 (0.01) & \textbf{-0.08 (0.01)} & \textbf{-0.04 (0.01)} & \textbf{-0.14 (0.01)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.04 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.09 (0.01)} & -0.02 (0.01) & 0.00 (0.01) & -0.06 (0.02)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.01 (0.00) & 0.00 (0.00) & -0.03 (0.00) & -0.03 (0.00) & -0.02 (0.00) & -0.05 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.02 (0.00) & 0.02 (0.00) & -0.07 (0.01) & \textbf{-0.06 (0.01)} & \textbf{-0.03 (0.00)} & \textbf{-0.12 (0.01)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.04 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.09 (0.01)} & -0.03 (0.00) & -0.01 (0.00) & -0.10 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & -0.01 (0.00) & 0.00 (0.00) & -0.03 (0.00) & -0.02 (0.00) & -0.01 (0.00) & -0.04 (0.00)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=1,k=1,4,12,sigma.sq=1,auto=TRUE.tex <==
\begin{table}
\centering
\caption{\label{tab:h=1, k=(1,4,12), sigma.sq=1, auto=TRUE}Mean rMSE per buckets of $\phi$ for $ h=1, k\in\{12,4,1\}, \sigma^2=1 $ and auto-selected models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrrr}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{3}{c}{Training rMSE} & \multicolumn{3}{c}{Test rMSE} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9}
Level & n & Recon. Type & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9] & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9]\\
\midrule
 &  & Bottom-Up & 0.00 (0.02) & 0.04 (0.01) & -0.02 (0.01) & \textbf{-0.06 (0.02)} & \textbf{-0.02 (0.01)} & 0.01 (0.04)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.07 (0.01)} & \textbf{-0.03 (0.00)} & \textbf{-0.12 (0.01)} & 0.00 (0.02) & 0.02 (0.01) & 0.07 (0.04)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.02 (0.00) & 0.00 (0.00) & -0.05 (0.00) & -0.04 (0.00) & -0.01 (0.00) & \textbf{-0.05 (0.01)}\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.02 (0.01) & 0.03 (0.01) & 0.00 (0.02) & \textbf{-0.07 (0.01)} & \textbf{-0.02 (0.01)} & \textbf{-0.08 (0.02)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.07 (0.01)} & \textbf{-0.02 (0.00)} & \textbf{-0.09 (0.01)} & -0.03 (0.01) & 0.01 (0.01) & -0.07 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.02 (0.00) & 0.00 (0.00) & -0.04 (0.00) & -0.03 (0.00) & -0.01 (0.00) & -0.06 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.02 (0.02) & 0.10 (0.02) & -0.04 (0.01) & \textbf{-0.04 (0.02)} & 0.06 (0.02) & -0.06 (0.02)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.06 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.10 (0.01)} & -0.04 (0.01) & 0.00 (0.01) & \textbf{-0.08 (0.01)}\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & -0.02 (0.00) & 0.00 (0.00) & -0.04 (0.00) & -0.03 (0.00) & \textbf{-0.01 (0.00)} & -0.05 (0.00)\\
\cmidrule{1-9}
 &  & Bottom-Up & -0.03 (0.01) & 0.01 (0.00) & 0.00 (0.01) & \textbf{-0.05 (0.01)} & \textbf{-0.02 (0.00)} & \textbf{-0.01 (0.01)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.06 (0.00)} & \textbf{-0.03 (0.00)} & \textbf{-0.07 (0.01)} & 0.00 (0.01) & 0.01 (0.01) & 0.06 (0.02)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.02 (0.00) & -0.01 (0.00) & 0.00 (0.01) & -0.01 (0.00) & 0.00 (0.00) & 0.03 (0.01)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.03 (0.00) & 0.01 (0.00) & 0.02 (0.01) & \textbf{-0.04 (0.01)} & \textbf{-0.01 (0.00)} & \textbf{-0.01 (0.01)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.05 (0.00)} & \textbf{-0.02 (0.00)} & \textbf{-0.04 (0.01)} & -0.01 (0.00) & 0.01 (0.00) & 0.05 (0.04)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.02 (0.00) & -0.01 (0.00) & 0.00 (0.00) & -0.01 (0.00) & 0.00 (0.00) & 0.05 (0.02)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.03 (0.00) & 0.02 (0.01) & 0.02 (0.01) & \textbf{-0.04 (0.00)} & 0.01 (0.01) & 0.01 (0.01)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.04 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.04 (0.00)} & -0.02 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.01)}\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & -0.02 (0.00) & -0.01 (0.00) & 0.02 (0.00) & -0.02 (0.00) & \textbf{ 0.00 (0.00)} & 0.04 (0.01)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.03 (0.00)} & \textbf{-0.02 (0.00)} & \textbf{-0.05 (0.01)} & 0.03 (0.01) & 0.02 (0.01) & 0.07 (0.02)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.01) & 0.01 (0.00) & 0.01 (0.00) & 0.05 (0.01)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.02 (0.00)} & \textbf{-0.02 (0.00)} & \textbf{-0.04 (0.01)} & 0.02 (0.00) & 0.01 (0.00) & 0.06 (0.04)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.01) & 0.00 (0.00) & 0.00 (0.00) & 0.06 (0.02)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & 0.00 (0.00) & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.01 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.04 (0.00)} & 0.01 (0.00) & 0.00 (0.00) & 0.00 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 3} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & -0.01 (0.00) & 0.01 (0.01) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & 0.03 (0.01)\\
\cmidrule{1-9}
 &  & Bottom-Up & -0.01 (0.01) & 0.03 (0.01) & -0.02 (0.01) & \textbf{-0.07 (0.01)} & \textbf{-0.02 (0.01)} & -0.01 (0.03)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.06 (0.01)} & \textbf{-0.03 (0.00)} & \textbf{-0.12 (0.01)} & -0.01 (0.01) & 0.01 (0.01) & 0.05 (0.03)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.02 (0.00) & -0.01 (0.00) & -0.05 (0.00) & -0.03 (0.00) & -0.01 (0.00) & \textbf{-0.05 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.02 (0.00) & 0.02 (0.01) & 0.00 (0.02) & \textbf{-0.05 (0.01)} & \textbf{-0.02 (0.01)} & \textbf{-0.08 (0.02)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.05 (0.00)} & \textbf{-0.02 (0.00)} & \textbf{-0.09 (0.01)} & -0.02 (0.01) & 0.00 (0.00) & -0.06 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.01 (0.00) & 0.00 (0.00) & -0.04 (0.00) & -0.02 (0.00) & -0.01 (0.00) & -0.05 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.01 (0.01) & 0.08 (0.02) & -0.03 (0.01) & \textbf{-0.04 (0.01)} & 0.05 (0.02) & -0.06 (0.02)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.04 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.10 (0.01)} & -0.03 (0.00) & 0.00 (0.00) & \textbf{-0.08 (0.01)}\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & -0.01 (0.00) & 0.00 (0.00) & -0.04 (0.00) & -0.02 (0.00) & \textbf{-0.01 (0.00)} & -0.04 (0.00)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=1,k=1,4,sigma.sq=1,auto=FALSE,name=test_rel_err.tex <==
\begin{table}
\centering
\caption{\label{tab:h=1, k=(1,4), sigma.sq=1, auto=FALSE, name=test_rel_err}Test mean rMSE per buckets of $\phi$ for $ h=1, k=(1,4), \sigma^2=1 $ and fixed order of the used models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrr}
\toprule
Level & n & Recon. Type & {}[-0.9,-0.6] & (-0.6,-0.3] & (-0.3,0.3] & (0.3,0.6] & (0.6,0.9]\\
\midrule
 &  & Bottom-Up & -0.079 (0.029) & -0.132 (0.041) & -0.060 (0.022) & -0.088 (0.029) & -0.121 (0.041)\\

 &  & Full Cov. & 0.070 (0.026) & 0.018 (0.029) & 0.053 (0.011) & 0.030 (0.021) & -0.046 (0.040)\\

 &  & Spectral & -0.028 (0.012) & -0.040 (0.027) & -0.034 (0.008) & -0.034 (0.019) & -0.090 (0.033)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.054 (0.006) & -0.063 (0.009) & -0.046 (0.005) & -0.052 (0.006) & -0.078 (0.008)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.089 (0.015) & -0.063 (0.017) & -0.064 (0.010) & -0.084 (0.014) & -0.176 (0.023)\\

 &  & Full Cov. & -0.057 (0.010) & -0.011 (0.010) & 0.016 (0.005) & -0.035 (0.011) & -0.149 (0.023)\\

 &  & Spectral & -0.052 (0.006) & -0.037 (0.006) & -0.033 (0.005) & -0.060 (0.009) & -0.174 (0.018)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.039 (0.003) & -0.028 (0.004) & -0.029 (0.003) & -0.037 (0.003) & -0.076 (0.005)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.096 (0.010) & -0.062 (0.012) & -0.034 (0.005) & -0.069 (0.008) & -0.179 (0.013)\\

 &  & Full Cov. & -0.071 (0.008) & -0.034 (0.008) & 0.004 (0.003) & -0.047 (0.007) & -0.165 (0.012)\\

 &  & Spectral & -0.060 (0.005) & -0.033 (0.006) & -0.020 (0.002) & -0.060 (0.006) & -0.169 (0.011)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & -0.038 (0.003) & -0.024 (0.003) & -0.014 (0.001) & -0.028 (0.002) & -0.070 (0.003)\\
\cmidrule{1-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & 0.158 (0.026) & 0.336 (0.137) & 0.192 (0.022) & 0.212 (0.035) & 0.172 (0.034)\\

 &  & Spectral & 0.032 (0.008) & 0.081 (0.031) & 0.057 (0.011) & 0.103 (0.020) & 0.126 (0.035)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.018 (0.005) & 0.036 (0.009) & 0.040 (0.008) & 0.093 (0.019) & 0.202 (0.037)\\
\cmidrule{2-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & 0.041 (0.007) & 0.047 (0.008) & 0.067 (0.010) & 0.063 (0.011) & 0.043 (0.008)\\

 &  & Spectral & 0.012 (0.002) & 0.014 (0.004) & 0.024 (0.007) & 0.030 (0.009) & 0.018 (0.006)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.008 (0.002) & 0.008 (0.002) & 0.020 (0.005) & 0.044 (0.008) & 0.136 (0.017)\\
\cmidrule{2-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & 0.015 (0.003) & 0.020 (0.004) & 0.022 (0.003) & 0.023 (0.003) & 0.019 (0.004)\\

 &  & Spectral & 0.007 (0.001) & 0.007 (0.002) & 0.006 (0.001) & 0.008 (0.002) & 0.013 (0.004)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & 0.007 (0.001) & 0.007 (0.002) & 0.006 (0.001) & 0.028 (0.004) & 0.110 (0.010)\\
\cmidrule{1-8}
 &  & Bottom-Up & -0.076 (0.014) & -0.122 (0.026) & -0.071 (0.015) & -0.094 (0.024) & -0.129 (0.035)\\

 &  & Full Cov. & 0.072 (0.014) & 0.062 (0.022) & 0.067 (0.010) & 0.037 (0.019) & -0.049 (0.035)\\

 &  & Spectral & -0.013 (0.007) & -0.031 (0.012) & -0.025 (0.006) & -0.030 (0.017) & -0.090 (0.029)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.031 (0.003) & -0.043 (0.005) & -0.035 (0.003) & -0.046 (0.004) & -0.071 (0.006)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.059 (0.009) & -0.048 (0.011) & -0.056 (0.009) & -0.078 (0.012) & -0.168 (0.020)\\

 &  & Full Cov. & -0.019 (0.006) & 0.005 (0.006) & 0.023 (0.005) & -0.028 (0.009) & -0.141 (0.021)\\

 &  & Spectral & -0.028 (0.003) & -0.021 (0.004) & -0.025 (0.005) & -0.053 (0.008) & -0.165 (0.016)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.022 (0.002) & -0.018 (0.002) & -0.022 (0.002) & -0.031 (0.003) & -0.066 (0.004)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.060 (0.006) & -0.044 (0.009) & -0.028 (0.004) & -0.063 (0.007) & -0.168 (0.012)\\

 &  & Full Cov. & -0.037 (0.005) & -0.017 (0.005) & 0.007 (0.003) & -0.040 (0.006) & -0.154 (0.011)\\

 &  & Spectral & -0.033 (0.003) & -0.021 (0.004) & -0.015 (0.002) & -0.054 (0.005) & -0.158 (0.010)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & -0.020 (0.001) & -0.015 (0.002) & -0.010 (0.001) & -0.023 (0.001) & -0.058 (0.002)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=1,k=1,4,sigma.sq=1,auto=FALSE,name=train_rel_err.tex <==
\begin{table}
\centering
\caption{\label{tab:h=1, k=(1,4), sigma.sq=1, auto=FALSE, name=train_rel_err}Training mean rMSE per buckets of $\phi$ for $ h=1, k=(1,4), \sigma^2=1 $ and fixed order of the used models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrr}
\toprule
Level & n & Recon. Type & {}[-0.9,-0.6] & (-0.6,-0.3] & (-0.3,0.3] & (0.3,0.6] & (0.6,0.9]\\
\midrule
 &  & Bottom-Up & 0.117 (0.015) & 0.132 (0.023) & 0.184 (0.012) & 0.135 (0.018) & -0.020 (0.020)\\

 &  & Full Cov. & -0.030 (0.007) & -0.027 (0.008) & 0.027 (0.011) & -0.044 (0.007) & -0.137 (0.012)\\

 &  & Spectral & -0.027 (0.004) & -0.017 (0.005) & 0.014 (0.002) & -0.022 (0.007) & -0.105 (0.013)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.012 (0.002) & -0.004 (0.003) & 0.009 (0.001) & -0.006 (0.003) & -0.047 (0.004)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.002 (0.008) & 0.033 (0.010) & 0.075 (0.005) & 0.010 (0.008) & -0.123 (0.011)\\

 &  & Full Cov. & -0.053 (0.004) & -0.025 (0.004) & -0.001 (0.002) & -0.048 (0.004) & -0.157 (0.008)\\

 &  & Spectral & -0.040 (0.004) & -0.017 (0.003) & 0.006 (0.001) & -0.039 (0.004) & -0.148 (0.008)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.019 (0.001) & -0.008 (0.001) & 0.003 (0.000) & -0.016 (0.001) & -0.061 (0.002)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.040 (0.004) & -0.002 (0.005) & 0.025 (0.002) & -0.030 (0.005) & -0.158 (0.008)\\

 &  & Full Cov. & -0.060 (0.003) & -0.026 (0.003) & -0.006 (0.001) & -0.052 (0.004) & -0.172 (0.007)\\

 &  & Spectral & -0.050 (0.003) & -0.021 (0.003) & -0.001 (0.001) & -0.047 (0.003) & -0.167 (0.007)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & -0.023 (0.001) & -0.011 (0.001) & -0.001 (0.000) & -0.019 (0.001) & -0.063 (0.002)\\
\cmidrule{1-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & -0.048 (0.006) & -0.061 (0.006) & -0.062 (0.008) & -0.094 (0.006) & -0.088 (0.007)\\

 &  & Spectral & -0.024 (0.002) & -0.031 (0.004) & -0.042 (0.003) & -0.065 (0.005) & -0.051 (0.007)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.008 (0.001) & -0.014 (0.002) & -0.032 (0.002) & -0.042 (0.006) & 0.011 (0.011)\\
\cmidrule{2-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & -0.020 (0.001) & -0.027 (0.002) & -0.032 (0.002) & -0.039 (0.002) & -0.031 (0.003)\\

 &  & Spectral & -0.010 (0.001) & -0.012 (0.002) & -0.019 (0.001) & -0.024 (0.002) & -0.018 (0.003)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.001 (0.000) & -0.004 (0.001) & -0.015 (0.001) & -0.006 (0.003) & 0.061 (0.007)\\
\cmidrule{2-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & -0.010 (0.001) & -0.015 (0.001) & -0.016 (0.001) & -0.017 (0.001) & -0.015 (0.001)\\

 &  & Spectral & -0.006 (0.001) & -0.005 (0.001) & -0.008 (0.001) & -0.009 (0.001) & -0.007 (0.001)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & 0.001 (0.000) & -0.001 (0.001) & -0.006 (0.001) & 0.008 (0.002) & 0.084 (0.006)\\
\cmidrule{1-8}
 &  & Bottom-Up & 0.053 (0.007) & 0.077 (0.012) & 0.131 (0.008) & 0.110 (0.015) & -0.023 (0.018)\\

 &  & Full Cov. & -0.039 (0.005) & -0.038 (0.005) & 0.003 (0.009) & -0.053 (0.006) & -0.136 (0.011)\\

 &  & Spectral & -0.026 (0.003) & -0.021 (0.004) & 0.000 (0.002) & -0.031 (0.006) & -0.104 (0.012)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.010 (0.001) & -0.007 (0.001) & -0.002 (0.001) & -0.013 (0.002) & -0.045 (0.003)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.003 (0.004) & 0.020 (0.006) & 0.056 (0.004) & 0.007 (0.007) & -0.115 (0.010)\\

 &  & Full Cov. & -0.039 (0.002) & -0.026 (0.003) & -0.008 (0.002) & -0.048 (0.004) & -0.149 (0.008)\\

 &  & Spectral & -0.027 (0.002) & -0.015 (0.002) & 0.000 (0.001) & -0.039 (0.004) & -0.139 (0.008)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.011 (0.001) & -0.007 (0.001) & -0.002 (0.000) & -0.015 (0.001) & -0.053 (0.002)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.022 (0.002) & -0.001 (0.003) & 0.020 (0.002) & -0.027 (0.004) & -0.147 (0.008)\\

 &  & Full Cov. & -0.038 (0.002) & -0.022 (0.002) & -0.008 (0.001) & -0.048 (0.003) & -0.161 (0.007)\\

 &  & Spectral & -0.030 (0.002) & -0.015 (0.002) & -0.003 (0.001) & -0.043 (0.003) & -0.156 (0.007)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & -0.012 (0.000) & -0.007 (0.000) & -0.002 (0.000) & -0.017 (0.001) & -0.053 (0.002)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=1,k=1,5,sigma.sq=1,auto=FALSE,name=test_rel_err.tex <==
\begin{table}
\centering
\caption{\label{tab:h=1, k=(1,5), sigma.sq=1, auto=FALSE, name=test_rel_err}Test mean rMSE per buckets of $\phi$ for $ h=1, k=(1,5), \sigma^2=1 $ and fixed order of the used models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrr}
\toprule
Level & n & Recon. Type & {}[-0.9,-0.6] & (-0.6,-0.3] & (-0.3,0.3] & (0.3,0.6] & (0.6,0.9]\\
\midrule
 &  & Bottom-Up & -0.151 (0.033) & -0.007 (0.040) & -0.063 (0.021) & -0.120 (0.031) & -0.227 (0.036)\\

 &  & Full Cov. & -0.045 (0.030) & 0.064 (0.039) & 0.102 (0.017) & -0.006 (0.018) & -0.081 (0.057)\\

 &  & Spectral & -0.089 (0.013) & -0.042 (0.013) & -0.011 (0.010) & -0.081 (0.017) & -0.180 (0.028)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.078 (0.006) & -0.030 (0.007) & -0.038 (0.004) & -0.050 (0.006) & -0.094 (0.007)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.178 (0.015) & -0.055 (0.019) & -0.067 (0.010) & -0.101 (0.013) & -0.206 (0.020)\\

 &  & Full Cov. & -0.143 (0.014) & -0.006 (0.013) & 0.025 (0.007) & -0.041 (0.011) & -0.191 (0.016)\\

 &  & Spectral & -0.114 (0.010) & -0.036 (0.007) & -0.033 (0.004) & -0.070 (0.010) & -0.200 (0.016)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.061 (0.003) & -0.025 (0.004) & -0.023 (0.002) & -0.035 (0.003) & -0.071 (0.004)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.178 (0.011) & -0.083 (0.013) & -0.032 (0.005) & -0.093 (0.009) & -0.181 (0.013)\\

 &  & Full Cov. & -0.164 (0.011) & -0.038 (0.008) & 0.000 (0.003) & -0.068 (0.007) & -0.173 (0.012)\\

 &  & Spectral & -0.148 (0.009) & -0.041 (0.008) & -0.019 (0.002) & -0.078 (0.007) & -0.176 (0.011)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & -0.057 (0.002) & -0.024 (0.003) & -0.010 (0.001) & -0.029 (0.002) & -0.061 (0.003)\\
\cmidrule{1-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & 0.196 (0.037) & 0.175 (0.061) & 0.262 (0.028) & 0.263 (0.039) & 0.262 (0.051)\\

 &  & Spectral & 0.066 (0.024) & 0.027 (0.015) & 0.088 (0.019) & 0.106 (0.028) & 0.150 (0.039)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.019 (0.004) & 0.014 (0.007) & 0.041 (0.008) & 0.100 (0.017) & 0.295 (0.041)\\
\cmidrule{2-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & 0.038 (0.008) & 0.048 (0.011) & 0.079 (0.012) & 0.060 (0.008) & 0.044 (0.011)\\

 &  & Spectral & 0.019 (0.004) & 0.013 (0.005) & 0.021 (0.005) & 0.025 (0.006) & 0.028 (0.011)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.011 (0.001) & 0.008 (0.002) & 0.018 (0.003) & 0.045 (0.006) & 0.159 (0.017)\\
\cmidrule{2-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & 0.013 (0.002) & 0.027 (0.007) & 0.019 (0.002) & 0.030 (0.005) & 0.015 (0.003)\\

 &  & Spectral & 0.008 (0.002) & 0.009 (0.003) & 0.003 (0.001) & 0.012 (0.003) & 0.011 (0.003)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & 0.009 (0.001) & 0.010 (0.003) & 0.005 (0.001) & 0.043 (0.008) & 0.115 (0.011)\\
\cmidrule{1-8}
 &  & Bottom-Up & -0.125 (0.018) & -0.032 (0.025) & -0.072 (0.016) & -0.120 (0.026) & -0.229 (0.032)\\

 &  & Full Cov. & -0.002 (0.017) & 0.049 (0.020) & 0.111 (0.015) & 0.007 (0.017) & -0.091 (0.042)\\

 &  & Spectral & -0.048 (0.009) & -0.030 (0.009) & -0.006 (0.009) & -0.072 (0.016) & -0.176 (0.026)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.047 (0.004) & -0.023 (0.004) & -0.032 (0.003) & -0.044 (0.004) & -0.083 (0.006)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.119 (0.009) & -0.048 (0.014) & -0.060 (0.009) & -0.095 (0.012) & -0.199 (0.019)\\

 &  & Full Cov. & -0.082 (0.008) & 0.005 (0.010) & 0.031 (0.007) & -0.034 (0.010) & -0.182 (0.016)\\

 &  & Spectral & -0.067 (0.006) & -0.025 (0.005) & -0.027 (0.003) & -0.064 (0.010) & -0.192 (0.015)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.035 (0.002) & -0.018 (0.003) & -0.019 (0.002) & -0.030 (0.002) & -0.063 (0.004)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.113 (0.007) & -0.063 (0.011) & -0.027 (0.004) & -0.086 (0.009) & -0.174 (0.013)\\

 &  & Full Cov. & -0.099 (0.007) & -0.022 (0.006) & 0.003 (0.002) & -0.061 (0.006) & -0.165 (0.011)\\

 &  & Spectral & -0.089 (0.006) & -0.029 (0.006) & -0.015 (0.002) & -0.072 (0.007) & -0.168 (0.011)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & -0.032 (0.001) & -0.017 (0.002) & -0.007 (0.001) & -0.024 (0.002) & -0.053 (0.002)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=1,k=1,5,sigma.sq=1,auto=FALSE,name=train_rel_err.tex <==
\begin{table}
\centering
\caption{\label{tab:h=1, k=(1,5), sigma.sq=1, auto=FALSE, name=train_rel_err}Training mean rMSE per buckets of $\phi$ for $ h=1, k=(1,5), \sigma^2=1 $ and fixed order of the used models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrr}
\toprule
Level & n & Recon. Type & {}[-0.9,-0.6] & (-0.6,-0.3] & (-0.3,0.3] & (0.3,0.6] & (0.6,0.9]\\
\midrule
 &  & Bottom-Up & 0.029 (0.020) & 0.148 (0.023) & 0.194 (0.012) & 0.141 (0.014) & -0.003 (0.022)\\

 &  & Full Cov. & -0.108 (0.012) & -0.014 (0.021) & 0.041 (0.022) & -0.018 (0.011) & -0.127 (0.011)\\

 &  & Spectral & -0.085 (0.008) & -0.020 (0.006) & 0.012 (0.002) & -0.008 (0.006) & -0.106 (0.012)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.040 (0.003) & -0.003 (0.003) & 0.007 (0.001) & -0.003 (0.002) & -0.043 (0.003)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.099 (0.010) & 0.033 (0.009) & 0.065 (0.005) & 0.004 (0.008) & -0.136 (0.011)\\

 &  & Full Cov. & -0.139 (0.008) & -0.029 (0.004) & -0.002 (0.001) & -0.048 (0.005) & -0.166 (0.008)\\

 &  & Spectral & -0.116 (0.008) & -0.021 (0.004) & 0.005 (0.001) & -0.039 (0.005) & -0.159 (0.008)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.047 (0.002) & -0.009 (0.001) & 0.001 (0.000) & -0.013 (0.001) & -0.054 (0.002)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.131 (0.008) & -0.006 (0.007) & 0.023 (0.002) & -0.018 (0.005) & -0.164 (0.009)\\

 &  & Full Cov. & -0.149 (0.007) & -0.035 (0.005) & -0.003 (0.002) & -0.042 (0.004) & -0.179 (0.008)\\

 &  & Spectral & -0.137 (0.007) & -0.029 (0.004) & 0.000 (0.001) & -0.037 (0.003) & -0.175 (0.008)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & -0.049 (0.002) & -0.010 (0.001) & 0.000 (0.000) & -0.014 (0.001) & -0.057 (0.002)\\
\cmidrule{1-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & -0.061 (0.006) & -0.032 (0.021) & -0.040 (0.015) & -0.088 (0.007) & -0.086 (0.006)\\

 &  & Spectral & -0.032 (0.004) & -0.027 (0.003) & -0.040 (0.002) & -0.059 (0.004) & -0.058 (0.006)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.002 (0.001) & -0.011 (0.002) & -0.025 (0.002) & -0.043 (0.004) & 0.008 (0.011)\\
\cmidrule{2-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & -0.026 (0.002) & -0.028 (0.002) & -0.029 (0.001) & -0.035 (0.002) & -0.029 (0.003)\\

 &  & Spectral & -0.015 (0.002) & -0.012 (0.002) & -0.014 (0.001) & -0.020 (0.002) & -0.016 (0.003)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.004 (0.001) & -0.003 (0.001) & -0.010 (0.001) & -0.003 (0.003) & 0.074 (0.008)\\
\cmidrule{2-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & -0.012 (0.001) & -0.014 (0.001) & -0.014 (0.001) & -0.017 (0.001) & -0.015 (0.001)\\

 &  & Spectral & -0.007 (0.001) & -0.007 (0.001) & -0.006 (0.000) & -0.009 (0.001) & -0.009 (0.001)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & 0.005 (0.000) & 0.000 (0.001) & -0.004 (0.000) & 0.004 (0.002) & 0.092 (0.007)\\
\cmidrule{1-8}
 &  & Bottom-Up & 0.005 (0.011) & 0.093 (0.014) & 0.144 (0.009) & 0.123 (0.012) & -0.007 (0.020)\\

 &  & Full Cov. & -0.092 (0.008) & -0.018 (0.021) & 0.021 (0.020) & -0.027 (0.010) & -0.126 (0.010)\\

 &  & Spectral & -0.066 (0.006) & -0.022 (0.004) & 0.001 (0.002) & -0.014 (0.005) & -0.105 (0.011)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.024 (0.001) & -0.005 (0.001) & 0.000 (0.001) & -0.008 (0.001) & -0.042 (0.003)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.060 (0.006) & 0.022 (0.006) & 0.051 (0.004) & 0.003 (0.007) & -0.130 (0.011)\\

 &  & Full Cov. & -0.094 (0.005) & -0.029 (0.003) & -0.008 (0.001) & -0.048 (0.004) & -0.160 (0.008)\\

 &  & Spectral & -0.076 (0.005) & -0.018 (0.003) & 0.001 (0.001) & -0.038 (0.004) & -0.152 (0.008)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.027 (0.001) & -0.007 (0.001) & -0.001 (0.000) & -0.013 (0.001) & -0.049 (0.002)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.079 (0.005) & -0.004 (0.004) & 0.018 (0.002) & -0.017 (0.004) & -0.157 (0.008)\\

 &  & Full Cov. & -0.095 (0.004) & -0.028 (0.003) & -0.005 (0.001) & -0.041 (0.003) & -0.171 (0.008)\\

 &  & Spectral & -0.086 (0.004) & -0.022 (0.003) & -0.001 (0.001) & -0.035 (0.003) & -0.167 (0.008)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & -0.027 (0.001) & -0.007 (0.001) & -0.001 (0.000) & -0.013 (0.001) & -0.050 (0.002)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=1,k=1,5,sigma.sq=1,auto=FALSE.tex <==
\begin{table}
\centering
\caption{\label{tab:h=1, k=(1,5), sigma.sq=1, auto=FALSE}Mean rMSE per buckets of $\phi$ for $ h=1, k\in\{5,1\}, \sigma^2=1 $ and fixed order of the used models. The standard errors are given in parentheses.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrrr}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{3}{c}{Training rMSE} & \multicolumn{3}{c}{Test rMSE} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9}
Level & n & Recon. Type & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9] & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9]\\
\midrule
 &  & Bottom-Up & 0.05 (0.02) & 0.17 (0.01) & 0.02 (0.02) & \textbf{-0.15 (0.03)} & \textbf{-0.09 (0.02)} & \textbf{-0.17 (0.02)}\\

 &  & Full Cov. & \textbf{-0.10 (0.01)} & 0.02 (0.01) & \textbf{-0.11 (0.01)} & 0.00 (0.04) & 0.07 (0.02) & -0.07 (0.02)\\

 &  & Spectral & -0.09 (0.01) & 0.01 (0.00) & -0.08 (0.01) & -0.08 (0.02) & 0.01 (0.01) & -0.11 (0.02)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.03 (0.00) & \textbf{ 0.00 (0.00)} & -0.03 (0.00) & -0.07 (0.00) & -0.04 (0.00) & -0.07 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.07 (0.01) & 0.06 (0.00) & -0.08 (0.01) & \textbf{-0.16 (0.01)} & \textbf{-0.07 (0.01)} & \textbf{-0.15 (0.02)}\\

 &  & Full Cov. & \textbf{-0.12 (0.01)} & \textbf{ 0.00 (0.01)} & \textbf{-0.12 (0.01)} & -0.14 (0.01) & 0.02 (0.01) & -0.12 (0.01)\\

 &  & Spectral & -0.10 (0.01) & 0.00 (0.00) & -0.10 (0.01) & -0.11 (0.01) & -0.02 (0.01) & -0.10 (0.02)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.04 (0.00) & 0.00 (0.00) & -0.04 (0.00) & -0.06 (0.00) & -0.02 (0.00) & -0.05 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.11 (0.01) & 0.02 (0.00) & -0.12 (0.01) & \textbf{-0.15 (0.01)} & \textbf{-0.05 (0.00)} & \textbf{-0.13 (0.01)}\\

 &  & Full Cov. & \textbf{-0.13 (0.01)} & \textbf{-0.01 (0.00)} & \textbf{-0.13 (0.01)} & -0.14 (0.01) & -0.01 (0.00) & -0.12 (0.01)\\

 &  & Spectral & -0.11 (0.01) & 0.00 (0.00) & -0.13 (0.01) & -0.12 (0.01) & -0.02 (0.00) & -0.12 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & -0.04 (0.00) & 0.00 (0.00) & -0.04 (0.00) & -0.05 (0.00) & -0.01 (0.00) & -0.05 (0.00)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.06 (0.00)} & \textbf{-0.06 (0.01)} & \textbf{-0.09 (0.01)} & 0.16 (0.02) & 0.21 (0.02) & 0.24 (0.03)\\

 &  & Spectral & -0.03 (0.00) & -0.04 (0.00) & -0.05 (0.01) & 0.07 (0.01) & 0.11 (0.02) & 0.16 (0.03)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & -0.03 (0.00) & 0.01 (0.01) & 0.02 (0.00) & 0.05 (0.01) & 0.21 (0.03)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.02 (0.00)} & \textbf{-0.03 (0.00)} & \textbf{-0.03 (0.00)} & 0.03 (0.00) & 0.07 (0.01) & 0.05 (0.01)\\

 &  & Spectral & -0.01 (0.00) & -0.02 (0.00) & -0.01 (0.00) & 0.01 (0.00) & 0.03 (0.01) & 0.06 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & -0.01 (0.00) & 0.04 (0.01) & 0.01 (0.00) & 0.02 (0.00) & 0.12 (0.01)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.01 (0.00)} & \textbf{-0.02 (0.00)} & \textbf{-0.01 (0.00)} & 0.01 (0.00) & 0.03 (0.00) & 0.01 (0.00)\\

 &  & Spectral & -0.01 (0.00) & -0.01 (0.00) & 0.00 (0.00) & 0.01 (0.00) & 0.01 (0.00) & 0.01 (0.00)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.06 (0.00) & 0.01 (0.00) & 0.01 (0.00) & 0.08 (0.01)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.02 (0.01) & 0.13 (0.01) & 0.02 (0.02) & \textbf{-0.13 (0.02)} & \textbf{-0.10 (0.01)} & \textbf{-0.17 (0.02)}\\

 &  & Full Cov. & \textbf{-0.09 (0.01)} & 0.00 (0.01) & \textbf{-0.11 (0.01)} & 0.02 (0.02) & 0.07 (0.01) & -0.06 (0.02)\\

 &  & Spectral & -0.07 (0.01) & 0.00 (0.00) & -0.08 (0.01) & -0.04 (0.01) & 0.01 (0.01) & -0.10 (0.02)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.02 (0.00) & \textbf{ 0.00 (0.00)} & -0.03 (0.00) & -0.04 (0.00) & -0.03 (0.00) & -0.06 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.05 (0.01) & 0.04 (0.00) & -0.08 (0.01) & \textbf{-0.11 (0.01)} & \textbf{-0.06 (0.01)} & \textbf{-0.15 (0.01)}\\

 &  & Full Cov. & \textbf{-0.08 (0.00)} & \textbf{-0.01 (0.01)} & \textbf{-0.12 (0.01)} & -0.08 (0.01) & 0.02 (0.01) & -0.11 (0.01)\\

 &  & Spectral & -0.07 (0.00) & 0.00 (0.00) & -0.10 (0.01) & -0.07 (0.01) & -0.02 (0.00) & -0.09 (0.02)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.02 (0.00) & 0.00 (0.00) & -0.04 (0.00) & -0.03 (0.00) & -0.02 (0.00) & -0.05 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.07 (0.00) & 0.02 (0.00) & -0.11 (0.01) & \textbf{-0.10 (0.01)} & \textbf{-0.04 (0.00)} & \textbf{-0.13 (0.01)}\\

 &  & Full Cov. & \textbf{-0.08 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.13 (0.01)} & -0.08 (0.01) & 0.00 (0.00) & -0.12 (0.01)\\

 &  & Spectral & -0.07 (0.00) & 0.00 (0.00) & -0.12 (0.01) & -0.07 (0.01) & -0.01 (0.00) & -0.11 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & -0.02 (0.00) & 0.00 (0.00) & -0.04 (0.00) & -0.03 (0.00) & -0.01 (0.00) & -0.04 (0.00)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=1,k=1,5,sigma.sq=1,auto=TRUE.tex <==
\begin{table}
\centering
\caption{\label{tab:h=1, k=(1,5), sigma.sq=1, auto=TRUE}Mean rMSE per buckets of $\phi$ for $ h=1, k\in\{5,1\}, \sigma^2=1 $ and auto-selected models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrrr}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{3}{c}{Training rMSE} & \multicolumn{3}{c}{Test rMSE} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9}
Level & n & Recon. Type & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9] & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9]\\
\midrule
 &  & Bottom-Up & -0.06 (0.02) & 0.04 (0.01) & -0.06 (0.02) & \textbf{-0.16 (0.03)} & -0.02 (0.01) & -0.05 (0.04)\\

 &  & Full Cov. & \textbf{-0.16 (0.01)} & - & \textbf{-0.18 (0.01)} & -0.08 (0.03) & - & -0.09 (0.03)\\

 &  & Spectral & -0.13 (0.01) & \textbf{-0.03 (0.00)} & -0.15 (0.01) & -0.09 (0.02) & -0.01 (0.01) & \textbf{-0.09 (0.02)}\\

 & \multirow{-4}{*}{ 20} & OLS & -0.05 (0.00) & -0.01 (0.00) & -0.07 (0.00) & -0.07 (0.00) & \textbf{-0.02 (0.00)} & -0.07 (0.01)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.10 (0.01) & 0.01 (0.00) & -0.10 (0.01) & \textbf{-0.15 (0.01)} & \textbf{-0.02 (0.01)} & \textbf{-0.17 (0.01)}\\

 &  & Full Cov. & \textbf{-0.14 (0.01)} & - & \textbf{-0.15 (0.01)} & -0.12 (0.01) & - & -0.15 (0.01)\\

 &  & Spectral & -0.12 (0.01) & \textbf{-0.02 (0.00)} & -0.13 (0.01) & -0.10 (0.01) & -0.01 (0.00) & -0.14 (0.02)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.04 (0.00) & 0.00 (0.00) & -0.05 (0.00) & -0.05 (0.00) & -0.01 (0.00) & -0.06 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.12 (0.01) & 0.01 (0.00) & -0.10 (0.01) & \textbf{-0.15 (0.01)} & \textbf{-0.03 (0.00)} & \textbf{-0.14 (0.01)}\\

 &  & Full Cov. & \textbf{-0.13 (0.01)} & - & \textbf{-0.13 (0.01)} & -0.13 (0.01) & - & -0.13 (0.01)\\

 &  & Spectral & -0.12 (0.01) & \textbf{-0.01 (0.00)} & -0.12 (0.01) & -0.11 (0.01) & -0.01 (0.00) & -0.12 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & -0.04 (0.00) & 0.00 (0.00) & -0.05 (0.00) & -0.05 (0.00) & -0.01 (0.00) & -0.05 (0.00)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.05 (0.00)} & - & \textbf{-0.09 (0.01)} & 0.09 (0.01) & - & 0.07 (0.02)\\

 &  & Spectral & -0.03 (0.00) & \textbf{-0.02 (0.00)} & -0.05 (0.01) & 0.04 (0.01) & 0.02 (0.01) & 0.06 (0.03)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & -0.01 (0.00) & 0.03 (0.01) & 0.01 (0.00) & 0.01 (0.00) & 0.12 (0.02)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.03 (0.00)} & - & \textbf{-0.04 (0.00)} & 0.03 (0.00) & - & 0.03 (0.01)\\

 &  & Spectral & -0.01 (0.00) & \textbf{-0.01 (0.00)} & -0.02 (0.00) & 0.02 (0.00) & 0.01 (0.00) & 0.03 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.05 (0.01) & 0.01 (0.00) & 0.00 (0.00) & 0.11 (0.01)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.01 (0.00)} & - & \textbf{-0.02 (0.00)} & 0.02 (0.00) & - & 0.01 (0.00)\\

 &  & Spectral & -0.01 (0.00) & \textbf{-0.01 (0.00)} & -0.01 (0.00) & 0.01 (0.00) & 0.01 (0.00) & 0.02 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.05 (0.00) & 0.01 (0.00) & 0.01 (0.00) & 0.08 (0.01)\\
\cmidrule{1-9}
 &  & Bottom-Up & -0.05 (0.01) & 0.03 (0.01) & -0.06 (0.02) & \textbf{-0.12 (0.01)} & \textbf{-0.02 (0.01)} & -0.07 (0.03)\\

 &  & Full Cov. & \textbf{-0.12 (0.01)} & - & \textbf{-0.18 (0.01)} & -0.03 (0.02) & - & -0.10 (0.02)\\

 &  & Spectral & -0.09 (0.01) & \textbf{-0.03 (0.00)} & -0.15 (0.01) & -0.05 (0.01) & -0.01 (0.01) & \textbf{-0.10 (0.02)}\\

 & \multirow{-4}{*}{ 20} & OLS & -0.03 (0.00) & -0.01 (0.00) & -0.06 (0.00) & -0.04 (0.00) & -0.01 (0.00) & -0.07 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.06 (0.01) & 0.01 (0.00) & -0.09 (0.01) & \textbf{-0.10 (0.01)} & \textbf{-0.02 (0.01)} & \textbf{-0.16 (0.01)}\\

 &  & Full Cov. & \textbf{-0.10 (0.01)} & - & \textbf{-0.14 (0.01)} & -0.07 (0.01) & - & -0.15 (0.01)\\

 &  & Spectral & -0.08 (0.00) & \textbf{-0.02 (0.00)} & -0.13 (0.01) & -0.06 (0.01) & -0.01 (0.00) & -0.13 (0.02)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.03 (0.00) & 0.00 (0.00) & -0.04 (0.00) & -0.03 (0.00) & -0.01 (0.00) & -0.05 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.07 (0.00) & 0.00 (0.00) & -0.10 (0.01) & \textbf{-0.10 (0.01)} & \textbf{-0.03 (0.00)} & \textbf{-0.13 (0.01)}\\

 &  & Full Cov. & \textbf{-0.09 (0.00)} & - & \textbf{-0.13 (0.01)} & -0.08 (0.01) & - & -0.12 (0.01)\\

 &  & Spectral & -0.07 (0.00) & \textbf{-0.01 (0.00)} & -0.12 (0.01) & -0.07 (0.01) & -0.01 (0.00) & -0.11 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & -0.02 (0.00) & 0.00 (0.00) & -0.04 (0.00) & -0.03 (0.00) & -0.01 (0.00) & -0.05 (0.00)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=2,k=1,12,sigma.sq=1,auto=FALSE.tex <==
\begin{table}
\centering
\caption{\label{tab:h=2, k=(1,12), sigma.sq=1, auto=FALSE}Mean rMSE per buckets of $\phi$ for $ h=2, k\in\{12,1\}, \sigma^2=1 $ and fixed order of the used models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrrr}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{3}{c}{Training rMSE} & \multicolumn{3}{c}{Test rMSE} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9}
Level & n & Recon. Type & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9] & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9]\\
\midrule
 &  & Bottom-Up & 0.03 (0.01) & 0.06 (0.00) & 0.02 (0.01) & \textbf{-0.02 (0.01)} & \textbf{-0.03 (0.01)} & 0.00 (0.02)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{ 0.00 (0.00)} & 0.00 (0.00) & \textbf{-0.03 (0.01)} & -0.01 (0.00) & -0.02 (0.00) & 0.02 (0.01)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & 0.00 (0.00) & -0.01 (0.00) & -0.01 (0.00) & \textbf{-0.01 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.02 (0.00) & 0.03 (0.00) & -0.01 (0.01) & \textbf{-0.02 (0.01)} & \textbf{-0.02 (0.00)} & \textbf{-0.01 (0.01)}\\

 &  & Full Cov. & \textbf{-0.01 (0.01)} & 0.02 (0.01) & \textbf{-0.05 (0.01)} & 0.04 (0.01) & 0.04 (0.01) & 0.05 (0.01)\\

 &  & Spectral & 0.00 (0.00) & 0.01 (0.00) & -0.05 (0.01) & -0.01 (0.00) & 0.00 (0.00) & 0.01 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.02 (0.00) & -0.03 (0.00) & \textbf{-0.02 (0.00)} & \textbf{-0.02 (0.00)} & \textbf{-0.01 (0.00)}\\

 &  & Full Cov. & \textbf{-0.02 (0.00)} & - & \textbf{-0.07 (0.01)} & 0.01 (0.00) & - & 0.04 (0.01)\\

 &  & Spectral & 0.00 (0.00) & 0.00 (0.00) & -0.06 (0.01) & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.01 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.03 (0.00)} & 0.00 (0.00) & 0.01 (0.00) & 0.04 (0.01)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.01) & 0.00 (0.00) & 0.00 (0.00) & 0.02 (0.01)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.05 (0.00)} & \textbf{-0.02 (0.00)} & \textbf{-0.05 (0.01)} & 0.08 (0.01) & 0.06 (0.01) & 0.06 (0.01)\\

 &  & Spectral & -0.01 (0.00) & -0.01 (0.00) & -0.03 (0.00) & 0.00 (0.00) & 0.01 (0.00) & 0.02 (0.00)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.02 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.05 (0.00)} & - & \textbf{-0.04 (0.00)} & 0.05 (0.01) & - & 0.05 (0.00)\\

 &  & Spectral & -0.01 (0.00) & \textbf{ 0.00 (0.00)} & -0.02 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.02 (0.00)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.02 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.00)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.02 (0.00) & 0.05 (0.00) & 0.02 (0.01) & \textbf{-0.03 (0.01)} & \textbf{-0.03 (0.01)} & \textbf{-0.01 (0.02)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.01 (0.00)} & 0.00 (0.00) & \textbf{-0.03 (0.01)} & -0.01 (0.00) & -0.01 (0.00) & 0.02 (0.01)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & 0.00 (0.00) & 0.00 (0.00) & -0.01 (0.00) & -0.01 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.01 (0.00) & 0.03 (0.00) & -0.01 (0.01) & \textbf{-0.01 (0.00)} & \textbf{-0.02 (0.00)} & \textbf{-0.01 (0.01)}\\

 &  & Full Cov. & \textbf{-0.02 (0.01)} & 0.01 (0.01) & \textbf{-0.05 (0.01)} & 0.05 (0.01) & 0.04 (0.01) & 0.05 (0.01)\\

 &  & Spectral & -0.01 (0.00) & 0.00 (0.00) & -0.05 (0.01) & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.02 (0.00) & -0.03 (0.00) & \textbf{-0.01 (0.00)} & \textbf{-0.02 (0.00)} & \textbf{-0.01 (0.00)}\\

 &  & Full Cov. & \textbf{-0.03 (0.00)} & - & \textbf{-0.07 (0.01)} & 0.03 (0.00) & - & 0.04 (0.01)\\

 &  & Spectral & 0.00 (0.00) & 0.00 (0.00) & -0.06 (0.01) & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=2,k=1,12,sigma.sq=1,auto=TRUE.tex <==
\begin{table}
\centering
\caption{\label{tab:h=2, k=(1,12), sigma.sq=1, auto=TRUE}Mean rMSE per buckets of $\phi$ for $ h=2, k\in\{12,1\}, \sigma^2=1 $ and auto-selected models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrrr}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{3}{c}{Training rMSE} & \multicolumn{3}{c}{Test rMSE} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9}
Level & n & Recon. Type & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9] & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9]\\
\midrule
 &  & Bottom-Up & 0.00 (0.01) & 0.02 (0.01) & -0.03 (0.02) & \textbf{ 0.00 (0.01)} & 0.02 (0.01) & 0.16 (0.05)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.01 (0.00)} & 0.00 (0.00) & \textbf{-0.08 (0.01)} & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & 0.09 (0.04)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & -0.02 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.01 (0.00) & 0.01 (0.01) & \textbf{-0.01 (0.01)} & \textbf{-0.01 (0.00)} & 0.19 (0.04)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.01 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.08 (0.01)} & 0.00 (0.00) & 0.00 (0.00) & 0.07 (0.02)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & 0.00 (0.00) & -0.02 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.03 (0.02) & 0.05 (0.01) & -0.02 (0.01) & 0.01 (0.02) & 0.03 (0.01) & 0.08 (0.02)\\

 &  & Full Cov. & \textbf{-0.06 (0.00)} & - & - & 0.04 (0.01) & - & -\\

 &  & Spectral & -0.01 (0.00) & 0.00 (0.00) & \textbf{-0.07 (0.01)} & \textbf{-0.01 (0.00)} & 0.00 (0.00) & 0.03 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & -0.01 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & 0.00 (0.00)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.01 (0.00)} & 0.00 (0.00) & \textbf{-0.03 (0.01)} & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.01)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & 0.04 (0.01) & 0.00 (0.00) & 0.00 (0.00) & \textbf{-0.01 (0.01)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & 0.00 (0.00)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.01 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.05 (0.01)} & 0.00 (0.00) & 0.00 (0.00) & -0.01 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.01) & 0.00 (0.00) & 0.00 (0.00) & \textbf{-0.04 (0.01)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00)\\

 &  & Full Cov. & \textbf{-0.08 (0.00)} & - & - & 0.08 (0.01) & - & -\\

 &  & Spectral & -0.01 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{-0.03 (0.00)} & 0.00 (0.00) & 0.00 (0.00) & -0.01 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.02 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.03 (0.01)}\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.02 (0.01) & -0.03 (0.02) & \textbf{ 0.00 (0.01)} & 0.01 (0.01) & 0.15 (0.05)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.01 (0.00)} & 0.00 (0.00) & \textbf{-0.08 (0.01)} & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & 0.09 (0.03)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & -0.02 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{-0.01 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.01 (0.00) & 0.00 (0.01) & \textbf{ 0.00 (0.00)} & \textbf{-0.01 (0.00)} & 0.18 (0.04)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.01 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.08 (0.01)} & 0.00 (0.00) & 0.00 (0.00) & 0.06 (0.02)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & 0.00 (0.00) & -0.02 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.02 (0.01) & 0.04 (0.01) & -0.02 (0.01) & 0.01 (0.01) & 0.03 (0.01) & 0.08 (0.02)\\

 &  & Full Cov. & \textbf{-0.07 (0.00)} & - & - & 0.05 (0.01) & - & -\\

 &  & Spectral & -0.01 (0.00) & 0.00 (0.00) & \textbf{-0.07 (0.01)} & \textbf{ 0.00 (0.00)} & 0.00 (0.00) & 0.03 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & -0.01 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=2,k=1,4,12,sigma.sq=1,auto=FALSE.tex <==
\begin{table}
\centering
\caption{\label{tab:h=2, k=(1,4,12), sigma.sq=1, auto=FALSE}Mean rMSE per buckets of $\phi$ for $ h=2, k\in\{12,4,1\}, \sigma^2=1 $ and fixed order of the used models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrrr}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{3}{c}{Training rMSE} & \multicolumn{3}{c}{Test rMSE} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9}
Level & n & Recon. Type & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9] & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9]\\
\midrule
 &  & Bottom-Up & 0.04 (0.01) & 0.06 (0.00) & 0.02 (0.01) & 0.01 (0.02) & \textbf{-0.03 (0.01)} & 0.00 (0.02)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.01 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.06 (0.01)} & 0.01 (0.01) & -0.01 (0.01) & 0.09 (0.05)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & 0.00 (0.00) & -0.01 (0.00) & \textbf{-0.01 (0.00)} & -0.02 (0.00) & \textbf{-0.02 (0.01)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.01 (0.00) & 0.03 (0.00) & -0.01 (0.01) & \textbf{-0.01 (0.01)} & \textbf{-0.02 (0.00)} & \textbf{-0.01 (0.01)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.02 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.06 (0.01)} & 0.00 (0.00) & 0.00 (0.00) & 0.03 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & 0.00 (0.00) & -0.01 (0.00) & -0.01 (0.00) & -0.01 (0.00) & -0.01 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.01 (0.00) & -0.03 (0.01) & \textbf{-0.01 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.01 (0.00)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.01 (0.00)} & 0.00 (0.00) & \textbf{-0.07 (0.01)} & 0.00 (0.00) & 0.00 (0.00) & 0.02 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & -0.01 (0.00) & 0.00 (0.00) & -0.01 (0.00) & -0.01 (0.00)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.01 (0.00) & 0.01 (0.00) & 0.01 (0.00) & 0.00 (0.01) & \textbf{ 0.00 (0.00)} & \textbf{ 0.01 (0.01)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.03 (0.00)} & \textbf{-0.02 (0.00)} & \textbf{-0.05 (0.01)} & 0.01 (0.01) & 0.01 (0.00) & 0.07 (0.03)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & -0.01 (0.00) & 0.01 (0.00) & \textbf{ 0.00 (0.00)} & 0.01 (0.00) & 0.02 (0.01)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.03 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.04 (0.00)} & 0.01 (0.00) & 0.01 (0.00) & 0.04 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.02 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.04 (0.00)} & 0.00 (0.00) & 0.01 (0.00) & 0.03 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.02 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.03 (0.00)} & \textbf{-0.02 (0.00)} & \textbf{-0.05 (0.01)} & 0.01 (0.01) & 0.01 (0.00) & 0.05 (0.02)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.01)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.02 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.04 (0.00)} & 0.01 (0.00) & 0.00 (0.00) & 0.03 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.02 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.03 (0.00)} & 0.01 (0.00) & 0.00 (0.00) & 0.03 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 3} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.02 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.02 (0.00) & 0.04 (0.00) & 0.02 (0.01) & -0.01 (0.01) & \textbf{-0.02 (0.01)} & -0.01 (0.01)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.02 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.06 (0.01)} & 0.01 (0.01) & -0.01 (0.00) & 0.07 (0.03)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & 0.00 (0.00) & -0.01 (0.00) & \textbf{-0.01 (0.00)} & -0.01 (0.00) & \textbf{-0.02 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.01 (0.00) & 0.02 (0.00) & -0.01 (0.01) & \textbf{-0.01 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.01 (0.01)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.02 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.06 (0.01)} & 0.01 (0.00) & 0.00 (0.00) & 0.03 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & 0.00 (0.00) & -0.01 (0.00) & -0.01 (0.00) & -0.01 (0.00) & -0.01 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.01 (0.00) & -0.03 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.01 (0.00)}\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.02 (0.00)} & 0.00 (0.00) & \textbf{-0.07 (0.01)} & 0.00 (0.00) & 0.00 (0.00) & 0.02 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & -0.01 (0.00) & 0.00 (0.00) & 0.00 (0.00) & -0.01 (0.00)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=2,k=1,4,12,sigma.sq=1,auto=TRUE.tex <==
\begin{table}
\centering
\caption{\label{tab:h=2, k=(1,4,12), sigma.sq=1, auto=TRUE}Mean rMSE per buckets of $\phi$ for $ h=2, k\in\{12,4,1\}, \sigma^2=1 $ and auto-selected models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrrr}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{3}{c}{Training rMSE} & \multicolumn{3}{c}{Test rMSE} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9}
Level & n & Recon. Type & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9] & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9]\\
\midrule
 &  & Bottom-Up & 0.00 (0.01) & -0.01 (0.00) & 0.00 (0.03) & \textbf{-0.02 (0.01)} & 0.01 (0.01) & 0.14 (0.05)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.03 (0.01)} & \textbf{-0.02 (0.00)} & \textbf{-0.12 (0.01)} & -0.01 (0.01) & 0.00 (0.00) & 0.13 (0.05)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & -0.01 (0.00) & -0.04 (0.01) & -0.01 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{-0.01 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.01 (0.01) & -0.01 (0.01) & \textbf{-0.01 (0.00)} & 0.00 (0.01) & 0.17 (0.04)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.02 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.10 (0.01)} & 0.01 (0.01) & 0.01 (0.00) & 0.05 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & 0.00 (0.00) & -0.03 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.05 (0.02) & 0.10 (0.02) & 0.00 (0.01) & 0.03 (0.02) & 0.08 (0.02) & 0.14 (0.03)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.02 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.09 (0.01)} & 0.00 (0.00) & 0.01 (0.00) & 0.04 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & 0.00 (0.00) & -0.02 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\
\cmidrule{1-9}
 &  & Bottom-Up & -0.01 (0.00) & 0.00 (0.00) & 0.01 (0.01) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & 0.03 (0.02)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.03 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.07 (0.01)} & 0.01 (0.00) & 0.00 (0.00) & 0.07 (0.03)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.02 (0.01) & 0.00 (0.00) & 0.00 (0.00) & \textbf{-0.01 (0.01)}\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.01 (0.00) & 0.00 (0.00) & 0.01 (0.01) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & 0.08 (0.02)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.04 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.06 (0.01)} & 0.02 (0.01) & 0.01 (0.00) & 0.03 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{-0.01 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.02 (0.01) & 0.01 (0.01) & 0.00 (0.00) & 0.02 (0.01) & 0.08 (0.02)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.03 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.06 (0.01)} & 0.01 (0.00) & 0.01 (0.00) & 0.04 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & 0.00 (0.00)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.03 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.06 (0.01)} & 0.01 (0.00) & 0.00 (0.00) & 0.03 (0.02)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.01) & 0.00 (0.00) & 0.00 (0.00) & \textbf{-0.02 (0.01)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & 0.00 (0.00)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.03 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.06 (0.01)} & 0.01 (0.00) & 0.01 (0.00) & -0.01 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.01) & 0.00 (0.00) & 0.00 (0.00) & \textbf{-0.04 (0.01)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.02 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.06 (0.01)} & 0.01 (0.00) & 0.00 (0.00) & -0.02 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 3} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & -0.01 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.05 (0.01)}\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.00 (0.00) & -0.01 (0.00) & -0.01 (0.02) & \textbf{-0.01 (0.00)} & 0.00 (0.00) & 0.12 (0.04)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.03 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.12 (0.01)} & 0.00 (0.00) & 0.00 (0.00) & 0.11 (0.05)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & 0.00 (0.00) & -0.04 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{-0.01 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.01 (0.00) & -0.01 (0.01) & \textbf{-0.01 (0.00)} & 0.00 (0.00) & 0.16 (0.03)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.03 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.09 (0.01)} & 0.01 (0.01) & 0.00 (0.00) & 0.05 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & 0.00 (0.00) & -0.03 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{-0.01 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.03 (0.02) & 0.07 (0.02) & 0.00 (0.01) & 0.02 (0.01) & 0.06 (0.02) & 0.13 (0.03)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.02 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.09 (0.01)} & 0.00 (0.00) & 0.01 (0.00) & 0.04 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & 0.00 (0.00) & -0.02 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.01 (0.00)}\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=2,k=1,4,sigma.sq=1,auto=FALSE,name=test_rel_err.tex <==
\begin{table}
\centering
\caption{\label{tab:h=2, k=(1,4), sigma.sq=1, auto=FALSE, name=test_rel_err}Test mean rMSE per buckets of $\phi$ for $ h=2, k=(1,4), \sigma^2=1 $ and fixed order of the used models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrr}
\toprule
Level & n & Recon. Type & {}[-0.9,-0.6] & (-0.6,-0.3] & (-0.3,0.3] & (0.3,0.6] & (0.6,0.9]\\
\midrule
 &  & Bottom-Up & -0.013 (0.016) & 0.005 (0.025) & -0.023 (0.012) & -0.002 (0.019) & 0.035 (0.057)\\

 &  & Full Cov. & 0.174 (0.049) & 0.174 (0.061) & 0.123 (0.031) & 0.152 (0.051) & 0.183 (0.065)\\

 &  & Spectral & -0.003 (0.008) & -0.007 (0.009) & -0.011 (0.006) & 0.010 (0.019) & 0.058 (0.046)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.014 (0.004) & -0.013 (0.005) & -0.015 (0.003) & -0.010 (0.004) & -0.024 (0.007)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.033 (0.009) & -0.028 (0.009) & -0.017 (0.005) & -0.019 (0.007) & -0.028 (0.009)\\

 &  & Full Cov. & 0.039 (0.015) & 0.038 (0.014) & 0.034 (0.010) & 0.049 (0.016) & 0.022 (0.018)\\

 &  & Spectral & -0.015 (0.004) & -0.009 (0.003) & -0.009 (0.002) & -0.008 (0.006) & -0.004 (0.014)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.014 (0.002) & -0.010 (0.002) & -0.008 (0.001) & -0.009 (0.002) & -0.015 (0.002)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.024 (0.005) & -0.028 (0.009) & -0.009 (0.003) & -0.008 (0.003) & -0.034 (0.007)\\

 &  & Full Cov. & 0.002 (0.007) & 0.013 (0.006) & 0.010 (0.003) & 0.011 (0.006) & 0.009 (0.012)\\

 &  & Spectral & -0.017 (0.003) & -0.012 (0.003) & -0.005 (0.001) & -0.007 (0.003) & -0.001 (0.011)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & -0.010 (0.001) & -0.009 (0.003) & -0.004 (0.001) & -0.004 (0.001) & -0.014 (0.001)\\
\cmidrule{1-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & 0.178 (0.027) & 0.219 (0.036) & 0.236 (0.040) & 0.173 (0.036) & 0.166 (0.030)\\

 &  & Spectral & 0.014 (0.006) & 0.006 (0.005) & 0.018 (0.005) & 0.021 (0.009) & 0.033 (0.011)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.002 (0.001) & 0.003 (0.003) & 0.010 (0.003) & 0.014 (0.007) & 0.065 (0.021)\\
\cmidrule{2-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & 0.103 (0.015) & 0.057 (0.013) & 0.054 (0.007) & 0.076 (0.016) & 0.040 (0.008)\\

 &  & Spectral & 0.010 (0.003) & 0.005 (0.002) & 0.005 (0.002) & 0.013 (0.006) & 0.017 (0.006)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.002 (0.001) & 0.003 (0.001) & 0.004 (0.001) & 0.009 (0.003) & 0.019 (0.006)\\
\cmidrule{2-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & 0.079 (0.009) & 0.038 (0.009) & 0.021 (0.003) & 0.024 (0.003) & 0.032 (0.005)\\

 &  & Spectral & 0.007 (0.003) & 0.005 (0.003) & 0.001 (0.001) & 0.002 (0.001) & 0.023 (0.004)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & 0.001 (0.000) & 0.005 (0.003) & 0.001 (0.001) & 0.003 (0.001) & 0.022 (0.005)\\
\cmidrule{1-8}
 &  & Bottom-Up & -0.017 (0.007) & -0.009 (0.013) & -0.023 (0.009) & -0.007 (0.016) & 0.005 (0.042)\\

 &  & Full Cov. & 0.124 (0.020) & 0.143 (0.028) & 0.124 (0.023) & 0.149 (0.047) & 0.151 (0.051)\\

 &  & Spectral & 0.000 (0.005) & -0.005 (0.006) & -0.007 (0.005) & 0.007 (0.017) & 0.034 (0.036)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.007 (0.001) & -0.008 (0.002) & -0.011 (0.002) & -0.010 (0.002) & -0.027 (0.005)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.018 (0.005) & -0.019 (0.006) & -0.015 (0.004) & -0.018 (0.006) & -0.027 (0.009)\\

 &  & Full Cov. & 0.064 (0.012) & 0.041 (0.010) & 0.038 (0.009) & 0.051 (0.015) & 0.022 (0.017)\\

 &  & Spectral & -0.003 (0.002) & -0.005 (0.002) & -0.007 (0.002) & -0.006 (0.006) & -0.004 (0.014)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.006 (0.001) & -0.006 (0.001) & -0.006 (0.001) & -0.008 (0.001) & -0.013 (0.002)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.011 (0.002) & -0.021 (0.007) & -0.007 (0.002) & -0.007 (0.003) & -0.032 (0.006)\\

 &  & Full Cov. & 0.041 (0.005) & 0.019 (0.005) & 0.012 (0.002) & 0.013 (0.006) & 0.010 (0.011)\\

 &  & Spectral & -0.003 (0.002) & -0.008 (0.002) & -0.004 (0.001) & -0.006 (0.003) & 0.000 (0.011)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & -0.004 (0.001) & -0.005 (0.002) & -0.003 (0.001) & -0.003 (0.001) & -0.012 (0.001)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=2,k=1,4,sigma.sq=1,auto=FALSE,name=train_rel_err.tex <==
\begin{table}
\centering
\caption{\label{tab:h=2, k=(1,4), sigma.sq=1, auto=FALSE, name=train_rel_err}Training mean rMSE per buckets of $\phi$ for $ h=2, k=(1,4), \sigma^2=1 $ and fixed order of the used models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrr}
\toprule
Level & n & Recon. Type & {}[-0.9,-0.6] & (-0.6,-0.3] & (-0.3,0.3] & (0.3,0.6] & (0.6,0.9]\\
\midrule
 &  & Bottom-Up & 0.023 (0.010) & 0.058 (0.009) & 0.064 (0.008) & 0.041 (0.008) & -0.161 (0.027)\\

 &  & Full Cov. & -0.031 (0.012) & 0.027 (0.046) & 0.058 (0.027) & 0.023 (0.015) & -0.194 (0.064)\\

 &  & Spectral & -0.021 (0.003) & -0.002 (0.002) & 0.000 (0.002) & -0.004 (0.005) & -0.238 (0.021)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.005 (0.002) & 0.003 (0.001) & 0.004 (0.001) & -0.001 (0.001) & -0.067 (0.005)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.017 (0.004) & 0.027 (0.005) & 0.031 (0.003) & 0.011 (0.004) & -0.242 (0.014)\\

 &  & Full Cov. & -0.041 (0.011) & -0.010 (0.003) & 0.024 (0.017) & -0.010 (0.015) & -0.302 (0.015)\\

 &  & Spectral & -0.026 (0.002) & 0.001 (0.001) & 0.004 (0.001) & -0.014 (0.003) & -0.293 (0.015)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.009 (0.001) & 0.002 (0.001) & 0.003 (0.000) & -0.002 (0.001) & -0.071 (0.004)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.030 (0.002) & 0.008 (0.002) & 0.013 (0.001) & -0.003 (0.002) & -0.260 (0.013)\\

 &  & Full Cov. & -0.051 (0.003) & -0.011 (0.003) & -0.001 (0.001) & -0.026 (0.005) & -0.324 (0.014)\\

 &  & Spectral & -0.027 (0.002) & 0.000 (0.000) & 0.002 (0.000) & -0.014 (0.002) & -0.319 (0.014)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & -0.010 (0.001) & 0.000 (0.000) & 0.001 (0.000) & -0.003 (0.000) & -0.074 (0.004)\\
\cmidrule{1-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & -0.098 (0.010) & -0.021 (0.051) & 0.009 (0.035) & -0.035 (0.016) & -0.073 (0.019)\\

 &  & Spectral & -0.032 (0.004) & -0.015 (0.002) & -0.021 (0.002) & -0.025 (0.003) & -0.062 (0.008)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.001 (0.000) & -0.006 (0.001) & -0.011 (0.001) & -0.012 (0.003) & 0.173 (0.023)\\
\cmidrule{2-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & -0.086 (0.007) & -0.037 (0.003) & -0.021 (0.004) & -0.028 (0.009) & -0.074 (0.005)\\

 &  & Spectral & -0.035 (0.003) & -0.010 (0.002) & -0.008 (0.001) & -0.017 (0.002) & -0.059 (0.005)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.000 (0.000) & -0.003 (0.001) & -0.006 (0.000) & -0.004 (0.002) & 0.208 (0.017)\\
\cmidrule{2-8}
 &  & Bottom-Up & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.000 (0.000)\\

 &  & Full Cov. & -0.098 (0.005) & -0.023 (0.002) & -0.014 (0.001) & -0.024 (0.003) & -0.074 (0.005)\\

 &  & Spectral & -0.044 (0.003) & -0.003 (0.000) & -0.003 (0.000) & -0.009 (0.001) & -0.066 (0.005)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & 0.001 (0.000) & -0.001 (0.000) & -0.003 (0.000) & 0.002 (0.001) & 0.219 (0.015)\\
\cmidrule{1-8}
 &  & Bottom-Up & 0.009 (0.004) & 0.036 (0.005) & 0.046 (0.005) & 0.034 (0.007) & -0.159 (0.024)\\

 &  & Full Cov. & -0.066 (0.009) & 0.010 (0.048) & 0.052 (0.029) & 0.013 (0.015) & -0.196 (0.056)\\

 &  & Spectral & -0.027 (0.003) & -0.006 (0.002) & -0.004 (0.002) & -0.008 (0.005) & -0.232 (0.020)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.003 (0.001) & 0.000 (0.001) & 0.001 (0.001) & -0.003 (0.001) & -0.058 (0.004)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.008 (0.002) & 0.018 (0.003) & 0.023 (0.002) & 0.009 (0.003) & -0.229 (0.013)\\

 &  & Full Cov. & -0.063 (0.009) & -0.019 (0.003) & 0.013 (0.014) & -0.012 (0.015) & -0.290 (0.015)\\

 &  & Spectral & -0.031 (0.002) & -0.003 (0.001) & 0.001 (0.000) & -0.015 (0.003) & -0.280 (0.014)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.004 (0.000) & 0.000 (0.000) & 0.001 (0.000) & -0.002 (0.000) & -0.057 (0.003)\\
\cmidrule{2-8}
 &  & Bottom-Up & -0.014 (0.001) & 0.006 (0.001) & 0.010 (0.001) & -0.003 (0.002) & -0.246 (0.012)\\

 &  & Full Cov. & -0.075 (0.003) & -0.015 (0.002) & -0.004 (0.001) & -0.026 (0.005) & -0.311 (0.013)\\

 &  & Spectral & -0.036 (0.002) & -0.001 (0.000) & 0.001 (0.000) & -0.014 (0.002) & -0.305 (0.013)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & -0.004 (0.000) & 0.000 (0.000) & 0.000 (0.000) & -0.002 (0.000) & -0.059 (0.003)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=2,k=1,4,sigma.sq=1,auto=FALSE.tex <==
\begin{table}
\centering
\caption{\label{tab:h=2, k=(1,4), sigma.sq=1, auto=FALSE}Mean rMSE per buckets of $\phi$ for $ h=2, k\in\{4,1\}, \sigma^2=1 $ and fixed order of the used models. The standard errors are given in parentheses.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrrr}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{3}{c}{Training rMSE} & \multicolumn{3}{c}{Test rMSE} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9}
Level & n & Recon. Type & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9] & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9]\\
\midrule
 &  & Bottom-Up & 0.02 (0.01) & 0.06 (0.00) & -0.11 (0.02) & -0.01 (0.02) & \textbf{-0.02 (0.01)} & 0.02 (0.02)\\

 &  & Full Cov. & 0.00 (0.02) & 0.02 (0.01) & -0.14 (0.03) & 0.18 (0.05) & 0.16 (0.03) & 0.21 (0.05)\\

 &  & Spectral & \textbf{-0.01 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.15 (0.02)} & -0.01 (0.01) & 0.00 (0.01) & 0.15 (0.05)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & 0.00 (0.00) & -0.04 (0.00) & \textbf{-0.01 (0.00)} & -0.01 (0.00) & \textbf{-0.01 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.01 (0.00) & 0.03 (0.00) & -0.14 (0.01) & \textbf{-0.04 (0.01)} & \textbf{-0.02 (0.01)} & \textbf{-0.04 (0.01)}\\

 &  & Full Cov. & \textbf{-0.04 (0.00)} & - & \textbf{-0.19 (0.01)} & 0.02 (0.01) & - & 0.01 (0.01)\\

 &  & Spectral & -0.02 (0.00) & 0.00 (0.00) & -0.17 (0.01) & -0.02 (0.00) & -0.01 (0.01) & -0.02 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.01 (0.00) & \textbf{ 0.00 (0.00)} & -0.04 (0.00) & -0.01 (0.00) & -0.01 (0.00) & -0.02 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.02 (0.00) & 0.01 (0.00) & -0.16 (0.01) & \textbf{-0.02 (0.00)} & \textbf{-0.02 (0.00)} & \textbf{-0.02 (0.01)}\\

 &  & Full Cov. & \textbf{-0.04 (0.00)} & 0.00 (0.00) & \textbf{-0.22 (0.01)} & 0.01 (0.01) & 0.01 (0.00) & 0.02 (0.01)\\

 &  & Spectral & -0.02 (0.00) & 0.00 (0.00) & -0.20 (0.01) & -0.02 (0.00) & 0.00 (0.00) & 0.01 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & -0.01 (0.00) & \textbf{ 0.00 (0.00)} & -0.05 (0.00) & -0.01 (0.00) & -0.01 (0.00) & -0.01 (0.00)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.08 (0.01)} & \textbf{-0.05 (0.01)} & \textbf{-0.06 (0.02)} & 0.18 (0.03) & 0.23 (0.03) & 0.13 (0.02)\\

 &  & Spectral & -0.03 (0.00) & -0.02 (0.00) & -0.04 (0.01) & 0.01 (0.00) & 0.03 (0.01) & 0.06 (0.01)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & -0.01 (0.00) & 0.12 (0.02) & 0.00 (0.00) & 0.01 (0.00) & 0.02 (0.01)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.09 (0.01)} & - & \textbf{-0.06 (0.00)} & 0.11 (0.01) & - & 0.04 (0.01)\\

 &  & Spectral & -0.03 (0.00) & \textbf{-0.01 (0.00)} & -0.04 (0.00) & 0.02 (0.00) & 0.01 (0.00) & 0.02 (0.00)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & -0.01 (0.00) & 0.12 (0.01) & 0.00 (0.00) & 0.01 (0.00) & 0.03 (0.01)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.09 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.06 (0.00)} & 0.08 (0.01) & 0.03 (0.00) & 0.03 (0.00)\\

 &  & Spectral & -0.04 (0.00) & 0.00 (0.00) & -0.04 (0.00) & 0.01 (0.00) & 0.01 (0.00) & 0.02 (0.00)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.14 (0.01) & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.00)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.01 (0.00) & 0.04 (0.00) & -0.11 (0.02) & \textbf{-0.01 (0.01)} & \textbf{-0.02 (0.01)} & 0.01 (0.02)\\

 &  & Full Cov. & \textbf{-0.04 (0.01)} & 0.00 (0.01) & -0.14 (0.03) & 0.12 (0.02) & 0.16 (0.02) & 0.18 (0.04)\\

 &  & Spectral & -0.02 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{-0.15 (0.02)} & 0.00 (0.00) & 0.00 (0.01) & 0.11 (0.04)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & 0.00 (0.00) & -0.04 (0.00) & -0.01 (0.00) & -0.01 (0.00) & \textbf{-0.01 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.02 (0.00) & -0.13 (0.01) & \textbf{-0.02 (0.00)} & \textbf{-0.02 (0.00)} & \textbf{-0.04 (0.01)}\\

 &  & Full Cov. & \textbf{-0.06 (0.00)} & - & \textbf{-0.19 (0.01)} & 0.06 (0.01) & - & 0.01 (0.01)\\

 &  & Spectral & -0.03 (0.00) & 0.00 (0.00) & -0.17 (0.01) & 0.00 (0.00) & 0.00 (0.00) & -0.02 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & -0.04 (0.00) & -0.01 (0.00) & -0.01 (0.00) & -0.01 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.01 (0.00) & 0.01 (0.00) & -0.15 (0.01) & \textbf{-0.01 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.02 (0.01)}\\

 &  & Full Cov. & \textbf{-0.07 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.21 (0.01)} & 0.04 (0.00) & 0.01 (0.00) & 0.02 (0.01)\\

 &  & Spectral & -0.03 (0.00) & 0.00 (0.00) & -0.19 (0.01) & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & 0.00 (0.00) & -0.04 (0.00) & 0.00 (0.00) & 0.00 (0.00) & -0.01 (0.00)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=2,k=1,4,sigma.sq=1,auto=TRUE.tex <==
\begin{table}
\centering
\caption{\label{tab:h=2, k=(1,4), sigma.sq=1, auto=TRUE}Mean rMSE per buckets of $\phi$ for $ h=2, k\in\{4,1\}, \sigma^2=1 $ and auto-selected models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrrr}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{3}{c}{Training rMSE} & \multicolumn{3}{c}{Test rMSE} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9}
Level & n & Recon. Type & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9] & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9]\\
\midrule
 &  & Bottom-Up & -0.02 (0.01) & 0.00 (0.00) & -0.16 (0.02) & 0.00 (0.02) & 0.02 (0.01) & 0.10 (0.03)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.04 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.21 (0.02)} & -0.01 (0.01) & 0.01 (0.01) & 0.06 (0.03)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.01 (0.00) & -0.01 (0.00) & -0.08 (0.01) & \textbf{-0.01 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.01 (0.01)}\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.02 (0.00) & 0.01 (0.00) & -0.18 (0.01) & \textbf{-0.02 (0.01)} & 0.00 (0.00) & 0.05 (0.02)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.03 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.21 (0.01)} & -0.01 (0.00) & 0.01 (0.00) & 0.05 (0.02)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.01 (0.00) & 0.00 (0.00) & -0.07 (0.01) & -0.01 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{-0.01 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.03 (0.00) & 0.01 (0.00) & -0.18 (0.01) & \textbf{-0.01 (0.00)} & \textbf{-0.01 (0.00)} & 0.03 (0.02)\\

 &  & Full Cov. & \textbf{-0.07 (0.00)} & - & \textbf{-0.25 (0.01)} & 0.04 (0.01) & - & 0.05 (0.01)\\

 &  & Spectral & -0.03 (0.00) & \textbf{ 0.00 (0.00)} & -0.22 (0.01) & -0.01 (0.00) & 0.00 (0.00) & 0.02 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & -0.01 (0.00) & 0.00 (0.00) & -0.07 (0.01) & -0.01 (0.00) & 0.00 (0.00) & \textbf{-0.01 (0.00)}\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & 0.00 (0.00)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.03 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.04 (0.01)} & 0.01 (0.01) & 0.01 (0.01) & 0.00 (0.01)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.15 (0.02) & 0.00 (0.00) & 0.00 (0.00) & \textbf{-0.01 (0.01)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & 0.00 (0.00) & 0.00 (0.00)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.04 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.03 (0.01)} & 0.01 (0.00) & 0.00 (0.00) & 0.02 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.15 (0.02) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{-0.02 (0.01)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & 0.00 (0.00)\\

 &  & Full Cov. & \textbf{-0.12 (0.00)} & - & \textbf{-0.07 (0.00)} & 0.09 (0.01) & - & 0.02 (0.01)\\

 &  & Spectral & -0.04 (0.00) & \textbf{ 0.00 (0.00)} & -0.04 (0.00) & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & 0.00 (0.00) & 0.14 (0.01) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.01)}\\
\cmidrule{1-9}
 &  & Bottom-Up & -0.01 (0.00) & 0.00 (0.00) & -0.15 (0.02) & \textbf{-0.01 (0.00)} & 0.00 (0.01) & 0.08 (0.03)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.04 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.20 (0.01)} & 0.00 (0.00) & 0.01 (0.01) & 0.05 (0.02)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.00 (0.00) & 0.00 (0.00) & -0.07 (0.01) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{-0.02 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.01 (0.00) & 0.00 (0.00) & -0.17 (0.01) & \textbf{-0.01 (0.00)} & 0.00 (0.00) & 0.04 (0.01)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.03 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.20 (0.01)} & 0.00 (0.00) & 0.00 (0.00) & 0.05 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.00 (0.00) & 0.00 (0.00) & -0.06 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{-0.02 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & -0.01 (0.00) & 0.01 (0.00) & -0.17 (0.01) & \textbf{-0.01 (0.00)} & \textbf{-0.01 (0.00)} & 0.02 (0.02)\\

 &  & Full Cov. & \textbf{-0.09 (0.00)} & - & \textbf{-0.24 (0.01)} & 0.06 (0.01) & - & 0.04 (0.01)\\

 &  & Spectral & -0.03 (0.00) & \textbf{ 0.00 (0.00)} & -0.21 (0.01) & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & 0.00 (0.00) & 0.00 (0.00) & -0.06 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{-0.01 (0.00)}\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=2,k=1,5,sigma.sq=1,auto=FALSE.tex <==
\begin{table}
\centering
\caption{\label{tab:h=2, k=(1,5), sigma.sq=1, auto=FALSE}Mean rMSE per buckets of $\phi$ for $ h=2, k\in\{5,1\}, \sigma^2=1 $ and fixed order of the used models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrrr}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{3}{c}{Training rMSE} & \multicolumn{3}{c}{Test rMSE} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9}
Level & n & Recon. Type & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9] & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9]\\
\midrule
 &  & Bottom-Up & 0.38 (0.05) & 0.07 (0.01) & -0.08 (0.01) & -0.02 (0.02) & 0.01 (0.01) & -0.02 (0.02)\\

 &  & Full Cov. & \textbf{-0.10 (0.01)} & 0.03 (0.01) & -0.11 (0.02) & 0.33 (0.06) & 0.15 (0.03) & 0.20 (0.06)\\

 &  & Spectral & -0.05 (0.01) & 0.00 (0.00) & \textbf{-0.12 (0.01)} & 0.04 (0.01) & 0.02 (0.03) & 0.07 (0.04)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.03 (0.00) & \textbf{ 0.00 (0.00)} & -0.03 (0.00) & \textbf{-0.02 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.02 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.31 (0.03) & 0.03 (0.00) & -0.11 (0.01) & \textbf{-0.04 (0.01)} & \textbf{-0.02 (0.00)} & \textbf{-0.03 (0.01)}\\

 &  & Full Cov. & \textbf{-0.08 (0.01)} & 0.01 (0.01) & \textbf{-0.16 (0.02)} & 0.15 (0.02) & 0.06 (0.01) & 0.05 (0.02)\\

 &  & Spectral & -0.05 (0.01) & 0.00 (0.00) & -0.15 (0.01) & 0.04 (0.01) & 0.01 (0.01) & 0.02 (0.02)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.03 (0.00) & \textbf{ 0.00 (0.00)} & -0.03 (0.00) & -0.01 (0.00) & -0.01 (0.00) & -0.01 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.29 (0.03) & 0.02 (0.00) & -0.13 (0.01) & \textbf{-0.03 (0.00)} & \textbf{-0.02 (0.00)} & \textbf{-0.02 (0.00)}\\

 &  & Full Cov. & \textbf{-0.09 (0.01)} & \textbf{ 0.00 (0.00)} & \textbf{-0.18 (0.01)} & 0.12 (0.01) & 0.01 (0.00) & 0.02 (0.01)\\

 &  & Spectral & -0.05 (0.01) & 0.00 (0.00) & -0.16 (0.01) & 0.04 (0.01) & 0.00 (0.00) & 0.00 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & 0.03 (0.00) & 0.00 (0.00) & -0.03 (0.00) & -0.01 (0.00) & -0.01 (0.00) & -0.01 (0.00)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.25 (0.01)} & \textbf{-0.03 (0.01)} & \textbf{-0.06 (0.01)} & 0.34 (0.06) & 0.21 (0.02) & 0.21 (0.03)\\

 &  & Spectral & -0.15 (0.01) & -0.02 (0.00) & -0.04 (0.01) & 0.04 (0.01) & 0.02 (0.00) & 0.07 (0.02)\\

 & \multirow{-4}{*}{ 20} & OLS & -0.01 (0.00) & -0.01 (0.00) & 0.09 (0.01) & 0.00 (0.00) & 0.01 (0.00) & 0.04 (0.01)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.23 (0.01)} & \textbf{-0.02 (0.00)} & \textbf{-0.06 (0.01)} & 0.18 (0.02) & 0.06 (0.01) & 0.05 (0.01)\\

 &  & Spectral & -0.18 (0.01) & -0.01 (0.00) & -0.03 (0.00) & 0.07 (0.01) & 0.02 (0.01) & 0.03 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.01 (0.00) & -0.01 (0.00) & 0.11 (0.01) & 0.00 (0.00) & 0.00 (0.00) & 0.02 (0.01)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)}\\

 &  & Full Cov. & \textbf{-0.23 (0.01)} & \textbf{-0.02 (0.00)} & \textbf{-0.05 (0.00)} & 0.16 (0.02) & 0.02 (0.00) & 0.03 (0.00)\\

 &  & Spectral & -0.18 (0.01) & 0.00 (0.00) & -0.03 (0.00) & 0.06 (0.01) & 0.01 (0.00) & 0.02 (0.00)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & -0.01 (0.00) & 0.00 (0.00) & 0.11 (0.01) & 0.00 (0.00) & 0.00 (0.00) & 0.01 (0.00)\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.13 (0.01) & 0.05 (0.00) & -0.08 (0.01) & \textbf{-0.03 (0.01)} & -0.01 (0.01) & \textbf{-0.02 (0.02)}\\

 &  & Full Cov. & \textbf{-0.18 (0.01)} & 0.02 (0.01) & -0.11 (0.02) & 0.27 (0.04) & 0.14 (0.02) & 0.18 (0.05)\\

 &  & Spectral & -0.11 (0.01) & \textbf{ 0.00 (0.00)} & \textbf{-0.12 (0.01)} & 0.03 (0.01) & 0.01 (0.01) & 0.06 (0.03)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.01 (0.00) & 0.00 (0.00) & -0.03 (0.00) & -0.01 (0.00) & \textbf{-0.01 (0.00)} & -0.02 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.12 (0.01) & 0.02 (0.00) & -0.11 (0.01) & \textbf{-0.03 (0.00)} & \textbf{-0.02 (0.00)} & \textbf{-0.03 (0.01)}\\

 &  & Full Cov. & \textbf{-0.17 (0.01)} & 0.01 (0.01) & \textbf{-0.16 (0.02)} & 0.16 (0.02) & 0.06 (0.01) & 0.05 (0.02)\\

 &  & Spectral & -0.13 (0.01) & 0.00 (0.00) & -0.14 (0.01) & 0.05 (0.01) & 0.01 (0.01) & 0.02 (0.02)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.01 (0.00) & \textbf{ 0.00 (0.00)} & -0.03 (0.00) & -0.01 (0.00) & -0.01 (0.00) & -0.01 (0.00)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.11 (0.01) & 0.01 (0.00) & -0.12 (0.01) & \textbf{-0.02 (0.00)} & \textbf{-0.01 (0.00)} & \textbf{-0.02 (0.00)}\\

 &  & Full Cov. & \textbf{-0.17 (0.01)} & \textbf{-0.01 (0.00)} & \textbf{-0.17 (0.01)} & 0.14 (0.01) & 0.01 (0.00) & 0.02 (0.01)\\

 &  & Spectral & -0.13 (0.01) & 0.00 (0.00) & -0.16 (0.01) & 0.05 (0.01) & 0.00 (0.00) & 0.00 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & 0.01 (0.00) & 0.00 (0.00) & -0.03 (0.00) & -0.01 (0.00) & 0.00 (0.00) & -0.01 (0.00)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/h=2,k=1,5,sigma.sq=1,auto=TRUE.tex <==
\begin{table}
\centering
\caption{\label{tab:h=2, k=(1,5), sigma.sq=1, auto=TRUE}Mean rMSE per buckets of $\phi$ for $ h=2, k\in\{5,1\}, \sigma^2=1 $ and auto-selected models. The standard errors are given in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lllrrrrrr}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{3}{c}{Training rMSE} & \multicolumn{3}{c}{Test rMSE} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9}
Level & n & Recon. Type & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9] & {}[-0.9,-0.5] & (-0.5,0.5] & (0.5,0.9]\\
\midrule
 &  & Bottom-Up & 0.30 (0.04) & 0.00 (0.00) & -0.11 (0.02) & 0.04 (0.02) & 0.03 (0.02) & 0.32 (0.17)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.06 (0.01)} & \textbf{-0.01 (0.01)} & \textbf{-0.19 (0.02)} & 0.03 (0.01) & 0.01 (0.01) & 0.06 (0.03)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.02 (0.00) & 0.00 (0.00) & -0.07 (0.01) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.01)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.32 (0.03) & 0.01 (0.00) & -0.14 (0.01) & \textbf{-0.02 (0.01)} & \textbf{ 0.00 (0.00)} & 0.04 (0.01)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.06 (0.01)} & \textbf{-0.01 (0.00)} & \textbf{-0.19 (0.01)} & 0.03 (0.00) & 0.00 (0.00) & 0.05 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.03 (0.00) & 0.00 (0.00) & -0.05 (0.00) & -0.01 (0.00) & 0.00 (0.00) & \textbf{-0.01 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.30 (0.03) & 0.01 (0.00) & -0.14 (0.01) & \textbf{-0.02 (0.01)} & \textbf{-0.01 (0.00)} & 0.01 (0.01)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.06 (0.01)} & \textbf{ 0.00 (0.00)} & \textbf{-0.18 (0.01)} & 0.04 (0.01) & 0.00 (0.00) & 0.03 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 1} & \multirow{-4}{*}{ 100} & OLS & 0.03 (0.00) & 0.00 (0.00) & -0.04 (0.00) & -0.01 (0.00) & 0.00 (0.00) & \textbf{-0.01 (0.00)}\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & 0.00 (0.00) & 0.00 (0.00)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.15 (0.01)} & \textbf{-0.01 (0.00)} & \textbf{-0.05 (0.01)} & 0.05 (0.02) & 0.00 (0.00) & \textbf{-0.02 (0.01)}\\

 & \multirow{-4}{*}{ 20} & OLS & -0.01 (0.00) & 0.00 (0.00) & 0.11 (0.02) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & 0.00 (0.02)\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & 0.00 (0.00)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.18 (0.01)} & \textbf{ 0.00 (0.00)} & \textbf{-0.04 (0.00)} & 0.06 (0.01) & 0.00 (0.00) & 0.01 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & -0.01 (0.00) & 0.00 (0.00) & 0.12 (0.01) & 0.00 (0.00) & 0.00 (0.00) & \textbf{-0.01 (0.01)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.00 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & 0.00 (0.00)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.18 (0.01)} & \textbf{ 0.00 (0.00)} & \textbf{-0.04 (0.00)} & 0.06 (0.01) & 0.00 (0.00) & 0.02 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Level 2} & \multirow{-4}{*}{ 100} & OLS & -0.01 (0.00) & 0.00 (0.00) & 0.11 (0.01) & 0.00 (0.00) & 0.00 (0.00) & \textbf{-0.01 (0.00)}\\
\cmidrule{1-9}
 &  & Bottom-Up & 0.10 (0.01) & 0.00 (0.00) & -0.11 (0.02) & 0.00 (0.01) & 0.02 (0.02) & 0.17 (0.07)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.12 (0.01)} & \textbf{-0.01 (0.00)} & \textbf{-0.18 (0.01)} & 0.03 (0.01) & 0.01 (0.01) & 0.04 (0.03)\\

 & \multirow{-4}{*}{ 20} & OLS & 0.01 (0.00) & 0.00 (0.00) & -0.07 (0.01) & \textbf{ 0.00 (0.00)} & \textbf{ 0.00 (0.00)} & \textbf{-0.02 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.11 (0.01) & 0.01 (0.00) & -0.14 (0.01) & \textbf{-0.02 (0.00)} & \textbf{ 0.00 (0.00)} & 0.04 (0.01)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.13 (0.01)} & \textbf{-0.01 (0.00)} & \textbf{-0.18 (0.01)} & 0.04 (0.01) & 0.00 (0.00) & 0.04 (0.01)\\

 & \multirow{-4}{*}{ 50} & OLS & 0.01 (0.00) & 0.00 (0.00) & -0.05 (0.00) & -0.01 (0.00) & 0.00 (0.00) & \textbf{-0.01 (0.00)}\\
\cmidrule{2-9}
 &  & Bottom-Up & 0.11 (0.01) & 0.01 (0.00) & -0.13 (0.01) & \textbf{-0.01 (0.00)} & \textbf{-0.01 (0.00)} & 0.01 (0.01)\\

 &  & Full Cov. & - & - & - & - & - & -\\

 &  & Spectral & \textbf{-0.13 (0.01)} & \textbf{ 0.00 (0.00)} & \textbf{-0.17 (0.01)} & 0.05 (0.01) & 0.00 (0.00) & 0.03 (0.01)\\

\multirow{-12}{*}[1\dimexpr\aboverulesep+\belowrulesep+\cmidrulewidth]{ Overall} & \multirow{-4}{*}{ 100} & OLS & 0.01 (0.00) & 0.00 (0.00) & -0.04 (0.00) & 0.00 (0.00) & 0.00 (0.00) & \textbf{-0.01 (0.00)}\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/test.tex <==
\begin{table}
    \centering
    \caption{\label{tab:dat_all}$10\%$-trimmed overall means for $5$ datasets and selected reconciliation methods. The standard errors are available in parenthesis.}
    \centering
    \resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
    \begin{tabular}[t]{llrrrrrrrrl}
    \toprule
    \multicolumn{3}{c}{ } & \multicolumn{4}{c}{Training rMSE} & \multicolumn{4}{c}{Test rMSE} \\
    \cmidrule(l{3pt}r{3pt}){4-7} \cmidrule(l{3pt}r{3pt}){8-11}
    Dataset & $n_b$ & $k\in$ & Bottom-Up & Full Cov. & OLS & Spectral & Bottom-Up & Full Cov. & OLS & Spectral\\
    \midrule
    Energy & 357-357 & $\{7,1\}$ & -0.03 (0.02) & -0.06 (0.01) & -0.02 (0.00) & -0.06 (0.01) & -0.02 (0.05) & -0.02 (0.05) & -0.02 (0.00) & -0.04 (0.03)\\
    Food & 35-535 & $\{5,1\}$ & 0.04 (0.01) & -0.03 (0.01) & -0.01 (0.00) & -0.01 (0.00) & 0.04 (0.02) & 0.01 (0.01) & -0.01 (0.00) & 0.00 (0.01)\\
    M3 & 32-72 & $\{5,1\}$ & -0.17 (0.02) & -0.28 (0.01) & -0.11 (0.00) & -0.27 (0.01) & -0.09 (0.03) & -0.13 (0.03) & -0.11 (0.01) & -0.19 (0.02)\\
    Prison & 48-48 & $\{4,1\}$ & -0.18 (0.12) & -0.12 (0.17) & -0.11 (0.02) & 0.00 (0.18) & -0.40 (0.12) & -0.30 (0.14) & -0.14 (0.03) & -0.01 (0.20)\\
    Tourism & 228-228 & $\{3,1\}$ & 0.03 (0.00) & -0.05 (0.00) & 0.00 (0.00) & -0.01 (0.00) & 0.01 (0.01) & -0.02 (0.01) & -0.01 (0.00) & -0.01 (0.00)\\
    \bottomrule
    \end{tabular}}
    \end{table}

==> tables_datex/dat_props_mae.tex <==
\begin{table}

\caption{\label{tab:dat_props}Dataset properties. $N$ denotes the number of total time series in the dataset, and $n_\text{bottom},n_\text{top}$ give the range of the available lengths in the hierarchy given by $k$.}
\centering
\begin{tabular}[t]{lllll}
\toprule
Dataset & $N$ & $n_{\text{bottom}}$ & $n_{\text{top}}$ & $k\in$\\
\midrule
Energy & 23 & 51-51 & 357-357 & $\{7,1\}$\\
Food & 122 & 10-107 & 50-535 & $\{5,1\}$\\
M3 & 756 & 9-18 & 36-72 & $\{4,1\}$\\
Prison & 8 & 12-12 & 48-48 & $\{4,1\}$\\
Tourism & 525 & 76-76 & 228-228 & $\{3,1\}$\\
\bottomrule
\end{tabular}
\end{table}


==> tables_datex/dat_res_rmae.tex <==
\begin{table}
\centering
\caption{\label{tab:dat_res}$10\%$-trimmed overall means for $5$ datasets and selected reconciliation methods. The standard errors are available in parenthesis.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lrrrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{4}{c}{Training rMSE} & \multicolumn{4}{c}{Test rMSE} \\
\cmidrule(l{3pt}r{3pt}){2-5} \cmidrule(l{3pt}r{3pt}){6-9}
Dataset & Bottom-Up & Full Cov. & OLS & Spectral & Bottom-Up & Full Cov. & OLS & Spectral\\
\midrule
Energy & -0.01 (0.01) & -0.02 (0.00) & 0.00 (0.00) & -0.02 (0.00) & -0.02 (0.01) & 0.00 (0.02) & 0.00 (0.01) & -0.02 (0.01)\\
Food & 0.01 (0.00) & -0.02 (0.00) & -0.01 (0.00) & -0.01 (0.00) & 0.02 (0.01) & 0.00 (0.01) & 0.00 (0.00) & -0.01 (0.00)\\
M3 & -0.07 (0.01) & -0.12 (0.01) & 0.01 (0.00) & -0.12 (0.01) & -0.08 (0.01) & -0.08 (0.01) & 0.01 (0.01) & -0.10 (0.01)\\
Prison & -0.09 (0.06) & -0.08 (0.08) & -0.01 (0.05) & -0.03 (0.08) & -0.16 (0.05) & -0.12 (0.09) & 0.07 (0.03) & 0.09 (0.14)\\
Tourism & 0.03 (0.00) & -0.02 (0.00) & -0.01 (0.00) & -0.02 (0.00) & 0.02 (0.01) & 0.00 (0.00) & -0.01 (0.00) & -0.01 (0.00)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables_datex/tot_add.tex <==
\begin{table}
\centering
\caption{\label{tab:data:ae:ta}Results for A\&E Total Addendances in a Month-Week Hierarchy with automatically selected base models.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lrrlrrrr}
\toprule
Level & Training Base MSE & Test Base MSE & Recon. Type & Training Recon. MSE & Test Recon. MSE & Training rMSE & Test rMSE\\
\midrule
 &  &  & Bottom-Up & 1219.43 & 1981.83 & 0.08 & -0.60\\

 &  &  & Full Cov. & 1116.95 & 3880.65 & -0.01 & -0.22\\

 &  &  & Spectral & 1121.99 & 3451.09 & -0.01 & -0.31\\

\multirow{-4}{*}{ Level 1} & \multirow{-4}{*}{ 1131.98} & \multirow{-4}{*}{ 4994.92} & OLS & 1117.96 & 4252.37 & -0.01 & -0.15\\
\cmidrule{1-8}
 &  &  & Bottom-Up & 150.19 & 170.12 & 0.00 & 0.00\\

 &  &  & Full Cov. & 144.19 & 302.58 & -0.04 & 0.78\\

 &  &  & Spectral & 144.28 & 269.33 & -0.04 & 0.58\\

\multirow{-4}{*}{ Level 2} & \multirow{-4}{*}{ 150.19} & \multirow{-4}{*}{ 170.12} & OLS & 145.96 & 317.58 & -0.03 & 0.87\\
\cmidrule{1-8}
 &  &  & Bottom-Up & 1369.62 & 2151.95 & 0.07 & -0.58\\

 &  &  & Full Cov. & 1261.13 & 4183.23 & -0.02 & -0.19\\

 &  &  & Spectral & 1266.27 & 3720.42 & -0.01 & -0.28\\

\multirow{-4}{*}{ Overall} & \multirow{-4}{*}{ 1282.17} & \multirow{-4}{*}{ 5165.04} & OLS & 1263.93 & 4569.95 & -0.01 & -0.12\\
\bottomrule
\end{tabular}}
\end{table}


==> tables_datex/tot_add2.tex <==
\begin{table}
\centering
\caption{\label{tab:data:ae:ta2}Results for A\&E Total Addendances in a month-week hierarchy with fixed-order models.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lrrlrrrr}
\toprule
Level & Training Base MSE & Test Base MSE & Recon. Type & Training Recon. MSE & Test Recon. MSE & Training rMSE & Test rMSE\\
\midrule
 &  &  & Bottom-Up & 1219.43 & 1981.83 & 0.08 & -0.09\\

 &  &  & Full Cov. & 1124.78 & 2222.40 & 0.00 & 0.03\\

 &  &  & Spectral & 1169.64 & 2021.56 & 0.04 & -0.07\\

\multirow{-4}{*}{ Level 1} & \multirow{-4}{*}{ 1125.60} & \multirow{-4}{*}{ 2166.15} & OLS & 1132.26 & 2112.09 & 0.01 & -0.02\\
\cmidrule{1-8}
 &  &  & Bottom-Up & 150.19 & 170.12 & 0.00 & 0.00\\

 &  &  & Full Cov. & 148.26 & 186.73 & -0.01 & 0.10\\

 &  &  & Spectral & 148.44 & 171.55 & -0.01 & 0.01\\

\multirow{-4}{*}{ Level 2} & \multirow{-4}{*}{ 150.19} & \multirow{-4}{*}{ 170.12} & OLS & 147.74 & 176.55 & -0.02 & 0.04\\
\cmidrule{1-8}
 &  &  & Bottom-Up & 1369.62 & 2151.95 & 0.07 & -0.08\\

 &  &  & Full Cov. & 1273.04 & 2409.12 & 0.00 & 0.03\\

 &  &  & Spectral & 1318.08 & 2193.11 & 0.03 & -0.06\\

\multirow{-4}{*}{ Overall} & \multirow{-4}{*}{ 1275.79} & \multirow{-4}{*}{ 2336.26} & OLS & 1280.00 & 2288.64 & 0.00 & -0.02\\
\bottomrule
\end{tabular}}
\end{table}


==> tables_datex/wool.tex <==
\begin{table}
\centering
\caption{\label{tab:data:wool}Results for the Wool Production Time Series in a Quarter-Biannual-Annual Hierarchy in units of $10^4$ tonnes and automatically selected models.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lrrlrrrr}
\toprule
Level & Training Base MSE & Test Base MSE & Recon. Type & Training Recon. MSE & Test Recon. MSE & Training rMSE & Test rMSE\\
\midrule
 &  &  & Bottom-Up & 156.23 & 293.50 & -0.35 & 0.45\\

 &  &  & Full Cov. & 135.64 & 542.48 & -0.44 & 1.67\\

 &  &  & Spectral & 145.64 & 342.42 & -0.40 & 0.69\\

\multirow{-4}{*}{ Level 1} & \multirow{-4}{*}{ 241.92} & \multirow{-4}{*}{ 202.84} & OLS & 206.32 & 206.05 & -0.15 & 0.02\\
\cmidrule{1-8}
 &  &  & Bottom-Up & 80.55 & 80.23 & -0.09 & 0.57\\

 &  &  & Full Cov. & 58.17 & 144.78 & -0.34 & 1.83\\

 &  &  & Spectral & 63.09 & 91.03 & -0.28 & 0.78\\

\multirow{-4}{*}{ Level 2} & \multirow{-4}{*}{ 88.15} & \multirow{-4}{*}{ 51.07} & OLS & 85.75 & 55.53 & -0.03 & 0.09\\
\cmidrule{1-8}
 &  &  & Bottom-Up & 24.59 & 23.54 & 0.00 & 0.00\\

 &  &  & Full Cov. & 18.65 & 39.17 & -0.24 & 0.66\\

 &  &  & Spectral & 19.90 & 25.79 & -0.19 & 0.10\\

\multirow{-4}{*}{ Level 3} & \multirow{-4}{*}{ 24.59} & \multirow{-4}{*}{ 23.54} & OLS & 25.89 & 17.36 & 0.05 & -0.26\\
\cmidrule{1-8}
 &  &  & Bottom-Up & 261.37 & 397.27 & -0.26 & 0.43\\

 &  &  & Full Cov. & 212.47 & 726.43 & -0.40 & 1.62\\

 &  &  & Spectral & 228.64 & 459.25 & -0.36 & 0.66\\

\multirow{-4}{*}{ Overall} & \multirow{-4}{*}{ 354.66} & \multirow{-4}{*}{ 277.45} & OLS & 317.96 & 278.94 & -0.10 & 0.01\\
\bottomrule
\end{tabular}}
\end{table}


==> tables_datex/wool2.tex <==
\begin{table}
\centering
\caption{\label{tab:data:wool2}Results for the Wool Production time series in a quarter-biannual-annual hierarchy in units of $10^4$ tonnes and fixed-order models.}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}[t]{lrrlrrrr}
\toprule
Level & Training Base MSE & Test Base MSE & Recon. Type & Training Recon. MSE & Test Recon. MSE & Training rMSE & Test rMSE\\
\midrule
 &  &  & Bottom-Up & 156.23 & 293.50 & 0.05 & 1.23\\

 &  &  & Full Cov. & 119.19 & 330.31 & -0.20 & 1.51\\

 &  &  & Spectral & 134.30 & 200.81 & -0.10 & 0.52\\

\multirow{-4}{*}{ Level 1} & \multirow{-4}{*}{ 149.18} & \multirow{-4}{*}{ 131.83} & OLS & 141.12 & 146.46 & -0.05 & 0.11\\
\cmidrule{1-8}
 &  &  & Bottom-Up & 80.55 & 80.23 & 0.07 & 1.11\\

 &  &  & Full Cov. & 50.70 & 87.30 & -0.33 & 1.30\\

 &  &  & Spectral & 59.84 & 53.83 & -0.21 & 0.42\\

\multirow{-4}{*}{ Level 2} & \multirow{-4}{*}{ 75.42} & \multirow{-4}{*}{ 37.98} & OLS & 66.77 & 40.65 & -0.11 & 0.07\\
\cmidrule{1-8}
 &  &  & Bottom-Up & 24.59 & 23.54 & 0.00 & 0.00\\

 &  &  & Full Cov. & 16.43 & 24.89 & -0.33 & 0.06\\

 &  &  & Spectral & 19.11 & 16.60 & -0.22 & -0.29\\

\multirow{-4}{*}{ Level 3} & \multirow{-4}{*}{ 24.59} & \multirow{-4}{*}{ 23.54} & OLS & 21.15 & 13.64 & -0.14 & -0.42\\
\cmidrule{1-8}
 &  &  & Bottom-Up & 261.37 & 397.27 & 0.05 & 1.05\\

 &  &  & Full Cov. & 186.32 & 442.49 & -0.25 & 1.29\\

 &  &  & Spectral & 213.25 & 271.25 & -0.14 & 0.40\\

\multirow{-4}{*}{ Overall} & \multirow{-4}{*}{ 249.19} & \multirow{-4}{*}{ 193.35} & OLS & 229.04 & 200.75 & -0.08 & 0.04\\
\bottomrule
\end{tabular}}
\end{table}

